A search for time-dependent astrophysical neutrino emission with IceCube data from 2012 to 2017

High-energy neutrinos are unique messengers of the high-energy universe, tracing the processes of cosmic-ray acceleration. This paper presents analyses focusing on time-dependent neutrino point-source searches. A scan of the whole sky, making no prior assumption about source candidates, is performed, looking for a space and time clustering of high-energy neutrinos in data collected by the IceCube Neutrino Observatory between 2012 and 2017. No statistically significant evidence for a time-dependent neutrino signal is found with this search during this period since all results are consistent with the background expectation. Within this study period, the blazar 3C 279, showed strong variability, inducing a very prominent gamma-ray flare observed in 2015 June. This event motivated a dedicated study of the blazar, which consists of searching for a time-dependent neutrino signal correlated with the gamma-ray emission. No evidence for a time-dependent signal is found. Hence, an upper limit on the neutrino fluence is derived, allowing us to constrain a hadronic emission model.

==> A search for time-dependent neutrino emission with IceCube data from 2012 to 2017_v8/acknowledgements.tex <==
The IceCube collaboration acknowledges the significant contributions to this manuscript from St\'ephanie Bron and Teresa Montaruli. The authors gratefully acknowledge the support from the following agencies and institutions:
USA {\textendash} U.S. National Science Foundation-Office of Polar Programs,
U.S. National Science Foundation-Physics Division,
Wisconsin Alumni Research Foundation,
Center for High Throughput Computing (CHTC) at the University of Wisconsin{\textendash}Madison,
Open Science Grid (OSG),
Extreme Science and Engineering Discovery Environment (XSEDE),
Frontera computing project at the Texas Advanced Computing Center,
U.S. Department of Energy-National Energy Research Scientific Computing Center,
Particle astrophysics research computing center at the University of Maryland,
Institute for Cyber-Enabled Research at Michigan State University,
and Astroparticle physics computational facility at Marquette University;
Belgium {\textendash} Funds for Scientific Research (FRS-FNRS and FWO),
FWO Odysseus and Big Science programmes,
and Belgian Federal Science Policy Office (Belspo);
Germany {\textendash} Bundesministerium f{\"u}r Bildung und Forschung (BMBF),
Deutsche Forschungsgemeinschaft (DFG),
Helmholtz Alliance for Astroparticle Physics (HAP),
Initiative and Networking Fund of the Helmholtz Association,
Deutsches Elektronen Synchrotron (DESY),
and High Performance Computing cluster of the RWTH Aachen;
Sweden {\textendash} Swedish Research Council,
Swedish Polar Research Secretariat,
Swedish National Infrastructure for Computing (SNIC),
and Knut and Alice Wallenberg Foundation;
Australia {\textendash} Australian Research Council;
Canada {\textendash} Natural Sciences and Engineering Research Council of Canada,
Calcul Qu{\'e}bec, Compute Ontario, Canada Foundation for Innovation, WestGrid, and Compute Canada;
Denmark {\textendash} Villum Fonden and Carlsberg Foundation;
New Zealand {\textendash} Marsden Fund;
Japan {\textendash} Japan Society for Promotion of Science (JSPS)
and Institute for Global Prominent Research (IGPR) of Chiba University;
Korea {\textendash} National Research Foundation of Korea (NRF);
Switzerland {\textendash} Swiss National Science Foundation (SNSF);
United Kingdom {\textendash} Department of Physics, University of Oxford.

==> A search for time-dependent neutrino emission with IceCube data from 2012 to 2017_v8/authorlist.tex <==
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\affiliation{Department of Physics, University of Adelaide, Adelaide, 5005, Australia}
\affiliation{Dept. of Physics and Astronomy, University of Alaska Anchorage, 3211 Providence Dr., Anchorage, AK 99508, USA}
\affiliation{Dept. of Physics, University of Texas at Arlington, 502 Yates St., Science Hall Rm 108, Box 19059, Arlington, TX 76019, USA}
\affiliation{CTSPS, Clark-Atlanta University, Atlanta, GA 30314, USA}
\affiliation{School of Physics and Center for Relativistic Astrophysics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\affiliation{Dept. of Physics, Southern University, Baton Rouge, LA 70813, USA}
\affiliation{Dept. of Physics, University of California, Berkeley, CA 94720, USA}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\affiliation{Institut f{\"u}r Physik, Humboldt-Universit{\"a}t zu Berlin, D-12489 Berlin, Germany}
\affiliation{Fakult{\"a}t f{\"u}r Physik {\&} Astronomie, Ruhr-Universit{\"a}t Bochum, D-44780 Bochum, Germany}
\affiliation{Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium}
\affiliation{Vrije Universiteit Brussel (VUB), Dienst ELEM, B-1050 Brussels, Belgium}
\affiliation{Department of Physics and Laboratory for Particle Physics and Cosmology, Harvard University, Cambridge, MA 02138, USA}
\affiliation{Dept. of Physics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation{Dept. of Physics and Institute for Global Prominent Research, Chiba University, Chiba 263-8522, Japan}
\affiliation{Department of Physics, Loyola University Chicago, Chicago, IL 60660, USA}
\affiliation{Dept. of Physics and Astronomy, University of Canterbury, Private Bag 4800, Christchurch, New Zealand}
\affiliation{Dept. of Physics, University of Maryland, College Park, MD 20742, USA}
\affiliation{Dept. of Astronomy, Ohio State University, Columbus, OH 43210, USA}
\affiliation{Dept. of Physics and Center for Cosmology and Astro-Particle Physics, Ohio State University, Columbus, OH 43210, USA}
\affiliation{Niels Bohr Institute, University of Copenhagen, DK-2100 Copenhagen, Denmark}
\affiliation{Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\affiliation{Dept. of Physics, University of Alberta, Edmonton, Alberta, Canada T6G 2E1}
\affiliation{Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, D-91058 Erlangen, Germany}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\affiliation{D{\'e}partement de physique nucl{\'e}aire et corpusculaire, Universit{\'e} de Gen{\`e}ve, CH-1211 Gen{\`e}ve, Switzerland}
\affiliation{Dept. of Physics and Astronomy, University of Gent, B-9000 Gent, Belgium}
\affiliation{Dept. of Physics and Astronomy, University of California, Irvine, CA 92697, USA}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\affiliation{Dept. of Physics and Astronomy, University of Kansas, Lawrence, KS 66045, USA}
\affiliation{SNOLAB, 1039 Regional Road 24, Creighton Mine 9, Lively, ON, Canada P3Y 1N2}
\affiliation{Department of Physics and Astronomy, UCLA, Los Angeles, CA 90095, USA}
\affiliation{Department of Physics, Mercer University, Macon, GA 31207-0001, USA}
\affiliation{Dept. of Astronomy, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\affiliation{Department of Physics, Marquette University, Milwaukee, WI, 53201, USA}
\affiliation{Institut f{\"u}r Kernphysik, Westf{\"a}lische Wilhelms-Universit{\"a}t M{\"u}nster, D-48149 M{\"u}nster, Germany}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\affiliation{Dept. of Physics, Yale University, New Haven, CT 06520, USA}
\affiliation{Dept. of Physics, University of Oxford, Parks Road, Oxford OX1 3PU, UK}
\affiliation{Dept. of Physics, Drexel University, 3141 Chestnut Street, Philadelphia, PA 19104, USA}
\affiliation{Physics Department, South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}
\affiliation{Dept. of Physics, University of Wisconsin, River Falls, WI 54022, USA}
\affiliation{Dept. of Physics and Astronomy, University of Rochester, Rochester, NY 14627, USA}
\affiliation{Oskar Klein Centre and Dept. of Physics, Stockholm University, SE-10691 Stockholm, Sweden}
\affiliation{Dept. of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794-3800, USA}
\affiliation{Dept. of Physics, Sungkyunkwan University, Suwon 16419, Korea}
\affiliation{Institute of Basic Science, Sungkyunkwan University, Suwon 16419, Korea}
\affiliation{Dept. of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\affiliation{Dept. of Astronomy and Astrophysics, Pennsylvania State University, University Park, PA 16802, USA}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\affiliation{Dept. of Physics and Astronomy, Uppsala University, Box 516, S-75120 Uppsala, Sweden}
\affiliation{Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany}
\affiliation{DESY, D-15738 Zeuthen, Germany}

\author{R. Abbasi}
\affiliation{Department of Physics, Loyola University Chicago, Chicago, IL 60660, USA}
\author{M. Ackermann}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{J. Adams}
\affiliation{Dept. of Physics and Astronomy, University of Canterbury, Private Bag 4800, Christchurch, New Zealand}
\author{J. A. Aguilar}
\affiliation{Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium}
\author{M. Ahlers}
\affiliation{Niels Bohr Institute, University of Copenhagen, DK-2100 Copenhagen, Denmark}
\author{M. Ahrens}
\affiliation{Oskar Klein Centre and Dept. of Physics, Stockholm University, SE-10691 Stockholm, Sweden}
\author{C. Alispach}
\affiliation{D{\'e}partement de physique nucl{\'e}aire et corpusculaire, Universit{\'e} de Gen{\`e}ve, CH-1211 Gen{\`e}ve, Switzerland}
\author{A. A. Alves Jr.}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{N. M. Amin}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{K. Andeen}
\affiliation{Department of Physics, Marquette University, Milwaukee, WI, 53201, USA}
\author{T. Anderson}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\author{I. Ansseau}
\affiliation{Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium}
\author{G. Anton}
\affiliation{Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, D-91058 Erlangen, Germany}
\author{C. Arg{\"u}elles}
\affiliation{Department of Physics and Laboratory for Particle Physics and Cosmology, Harvard University, Cambridge, MA 02138, USA}
\author{S. Axani}
\affiliation{Dept. of Physics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{X. Bai}
\affiliation{Physics Department, South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}
\author{A. Balagopal V.}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{A. Barbano}
\affiliation{D{\'e}partement de physique nucl{\'e}aire et corpusculaire, Universit{\'e} de Gen{\`e}ve, CH-1211 Gen{\`e}ve, Switzerland}
\author{S. W. Barwick}
\affiliation{Dept. of Physics and Astronomy, University of California, Irvine, CA 92697, USA}
\author{B. Bastian}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{V. Basu}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{V. Baum}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{S. Baur}
\affiliation{Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium}
\author{R. Bay}
\affiliation{Dept. of Physics, University of California, Berkeley, CA 94720, USA}
\author{J. J. Beatty}
\affiliation{Dept. of Astronomy, Ohio State University, Columbus, OH 43210, USA}
\affiliation{Dept. of Physics and Center for Cosmology and Astro-Particle Physics, Ohio State University, Columbus, OH 43210, USA}
\author{K.-H. Becker}
\affiliation{Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany}
\author{J. Becker Tjus}
\affiliation{Fakult{\"a}t f{\"u}r Physik {\&} Astronomie, Ruhr-Universit{\"a}t Bochum, D-44780 Bochum, Germany}
\author{C. Bellenghi}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{S. BenZvi}
\affiliation{Dept. of Physics and Astronomy, University of Rochester, Rochester, NY 14627, USA}
\author{D. Berley}
\affiliation{Dept. of Physics, University of Maryland, College Park, MD 20742, USA}
\author{E. Bernardini}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\thanks{also at Universit{\`a} di Padova, I-35131 Padova, Italy}
\author{D. Z. Besson}
\affiliation{Dept. of Physics and Astronomy, University of Kansas, Lawrence, KS 66045, USA}
\thanks{also at National Research Nuclear University, Moscow Engineering Physics Institute (MEPhI), Moscow 115409, Russia}
\author{G. Binder}
\affiliation{Dept. of Physics, University of California, Berkeley, CA 94720, USA}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\author{D. Bindig}
\affiliation{Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany}
\author{E. Blaufuss}
\affiliation{Dept. of Physics, University of Maryland, College Park, MD 20742, USA}
\author{S. Blot}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{S. B{\"o}ser}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{O. Botner}
\affiliation{Dept. of Physics and Astronomy, Uppsala University, Box 516, S-75120 Uppsala, Sweden}
\author{J. B{\"o}ttcher}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{E. Bourbeau}
\affiliation{Niels Bohr Institute, University of Copenhagen, DK-2100 Copenhagen, Denmark}
\author{J. Bourbeau}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{F. Bradascio}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{J. Braun}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{S. Bron}
\affiliation{D{\'e}partement de physique nucl{\'e}aire et corpusculaire, Universit{\'e} de Gen{\`e}ve, CH-1211 Gen{\`e}ve, Switzerland}
\author{J. Brostean-Kaiser}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{A. Burgman}
\affiliation{Dept. of Physics and Astronomy, Uppsala University, Box 516, S-75120 Uppsala, Sweden}
\author{R. S. Busse}
\affiliation{Institut f{\"u}r Kernphysik, Westf{\"a}lische Wilhelms-Universit{\"a}t M{\"u}nster, D-48149 M{\"u}nster, Germany}
\author{M. A. Campana}
\affiliation{Dept. of Physics, Drexel University, 3141 Chestnut Street, Philadelphia, PA 19104, USA}
\author{C. Chen}
\affiliation{School of Physics and Center for Relativistic Astrophysics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\author{D. Chirkin}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{S. Choi}
\affiliation{Dept. of Physics, Sungkyunkwan University, Suwon 16419, Korea}
\author{B. A. Clark}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{K. Clark}
\affiliation{SNOLAB, 1039 Regional Road 24, Creighton Mine 9, Lively, ON, Canada P3Y 1N2}
\author{L. Classen}
\affiliation{Institut f{\"u}r Kernphysik, Westf{\"a}lische Wilhelms-Universit{\"a}t M{\"u}nster, D-48149 M{\"u}nster, Germany}
\author{A. Coleman}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{G. H. Collin}
\affiliation{Dept. of Physics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{J. M. Conrad}
\affiliation{Dept. of Physics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{P. Coppin}
\affiliation{Vrije Universiteit Brussel (VUB), Dienst ELEM, B-1050 Brussels, Belgium}
\author{P. Correa}
\affiliation{Vrije Universiteit Brussel (VUB), Dienst ELEM, B-1050 Brussels, Belgium}
\author{D. F. Cowen}
\affiliation{Dept. of Astronomy and Astrophysics, Pennsylvania State University, University Park, PA 16802, USA}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\author{R. Cross}
\affiliation{Dept. of Physics and Astronomy, University of Rochester, Rochester, NY 14627, USA}
\author{P. Dave}
\affiliation{School of Physics and Center for Relativistic Astrophysics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\author{C. De Clercq}
\affiliation{Vrije Universiteit Brussel (VUB), Dienst ELEM, B-1050 Brussels, Belgium}
\author{J. J. DeLaunay}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\author{H. Dembinski}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{K. Deoskar}
\affiliation{Oskar Klein Centre and Dept. of Physics, Stockholm University, SE-10691 Stockholm, Sweden}
\author{S. De Ridder}
\affiliation{Dept. of Physics and Astronomy, University of Gent, B-9000 Gent, Belgium}
\author{A. Desai}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{P. Desiati}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{K. D. de Vries}
\affiliation{Vrije Universiteit Brussel (VUB), Dienst ELEM, B-1050 Brussels, Belgium}
\author{G. de Wasseige}
\affiliation{Vrije Universiteit Brussel (VUB), Dienst ELEM, B-1050 Brussels, Belgium}
\author{M. de With}
\affiliation{Institut f{\"u}r Physik, Humboldt-Universit{\"a}t zu Berlin, D-12489 Berlin, Germany}
\author{T. DeYoung}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{S. Dharani}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{A. Diaz}
\affiliation{Dept. of Physics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{J. C. D{\'\i}az-V{\'e}lez}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{H. Dujmovic}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{M. Dunkman}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\author{M. A. DuVernois}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{E. Dvorak}
\affiliation{Physics Department, South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}
\author{T. Ehrhardt}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{P. Eller}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{R. Engel}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{J. Evans}
\affiliation{Dept. of Physics, University of Maryland, College Park, MD 20742, USA}
\author{P. A. Evenson}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{S. Fahey}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{A. R. Fazely}
\affiliation{Dept. of Physics, Southern University, Baton Rouge, LA 70813, USA}
\author{S. Fiedlschuster}
\affiliation{Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, D-91058 Erlangen, Germany}
\author{A.T. Fienberg}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\author{K. Filimonov}
\affiliation{Dept. of Physics, University of California, Berkeley, CA 94720, USA}
\author{C. Finley}
\affiliation{Oskar Klein Centre and Dept. of Physics, Stockholm University, SE-10691 Stockholm, Sweden}
\author{L. Fischer}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{D. Fox}
\affiliation{Dept. of Astronomy and Astrophysics, Pennsylvania State University, University Park, PA 16802, USA}
\author{A. Franckowiak}
\affiliation{Fakult{\"a}t f{\"u}r Physik {\&} Astronomie, Ruhr-Universit{\"a}t Bochum, D-44780 Bochum, Germany}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{E. Friedman}
\affiliation{Dept. of Physics, University of Maryland, College Park, MD 20742, USA}
\author{A. Fritz}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{P. F{\"u}rst}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{T. K. Gaisser}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{J. Gallagher}
\affiliation{Dept. of Astronomy, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{E. Ganster}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{S. Garrappa}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{L. Gerhardt}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\author{A. Ghadimi}
\affiliation{Dept. of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\author{C. Glaser}
\affiliation{Dept. of Physics and Astronomy, Uppsala University, Box 516, S-75120 Uppsala, Sweden}
\author{T. Glauch}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{T. Gl{\"u}senkamp}
\affiliation{Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, D-91058 Erlangen, Germany}
\author{A. Goldschmidt}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\author{J. G. Gonzalez}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{S. Goswami}
\affiliation{Dept. of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\author{D. Grant}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{T. Gr{\'e}goire}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\author{Z. Griffith}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{S. Griswold}
\affiliation{Dept. of Physics and Astronomy, University of Rochester, Rochester, NY 14627, USA}
\author{M. G{\"u}nd{\"u}z}
\affiliation{Fakult{\"a}t f{\"u}r Physik {\&} Astronomie, Ruhr-Universit{\"a}t Bochum, D-44780 Bochum, Germany}
\author{C. Haack}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{A. Hallgren}
\affiliation{Dept. of Physics and Astronomy, Uppsala University, Box 516, S-75120 Uppsala, Sweden}
\author{R. Halliday}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{L. Halve}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{F. Halzen}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{M. Ha Minh}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{K. Hanson}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{J. Hardin}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{A. A. Harnisch}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{A. Haungs}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{S. Hauser}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{D. Hebecker}
\affiliation{Institut f{\"u}r Physik, Humboldt-Universit{\"a}t zu Berlin, D-12489 Berlin, Germany}
\author{K. Helbing}
\affiliation{Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany}
\author{F. Henningsen}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{E. C. Hettinger}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{S. Hickford}
\affiliation{Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany}
\author{J. Hignight}
\affiliation{Dept. of Physics, University of Alberta, Edmonton, Alberta, Canada T6G 2E1}
\author{C. Hill}
\affiliation{Dept. of Physics and Institute for Global Prominent Research, Chiba University, Chiba 263-8522, Japan}
\author{G. C. Hill}
\affiliation{Department of Physics, University of Adelaide, Adelaide, 5005, Australia}
\author{K. D. Hoffman}
\affiliation{Dept. of Physics, University of Maryland, College Park, MD 20742, USA}
\author{R. Hoffmann}
\affiliation{Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany}
\author{T. Hoinka}
\affiliation{Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany}
\author{B. Hokanson-Fasig}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{K. Hoshina}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\thanks{also at Earthquake Research Institute, University of Tokyo, Bunkyo, Tokyo 113-0032, Japan}
\author{F. Huang}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\author{M. Huber}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{T. Huber}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{K. Hultqvist}
\affiliation{Oskar Klein Centre and Dept. of Physics, Stockholm University, SE-10691 Stockholm, Sweden}
\author{M. H{\"u}nnefeld}
\affiliation{Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany}
\author{R. Hussain}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{S. In}
\affiliation{Dept. of Physics, Sungkyunkwan University, Suwon 16419, Korea}
\author{N. Iovine}
\affiliation{Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium}
\author{A. Ishihara}
\affiliation{Dept. of Physics and Institute for Global Prominent Research, Chiba University, Chiba 263-8522, Japan}
\author{M. Jansson}
\affiliation{Oskar Klein Centre and Dept. of Physics, Stockholm University, SE-10691 Stockholm, Sweden}
\author{G. S. Japaridze}
\affiliation{CTSPS, Clark-Atlanta University, Atlanta, GA 30314, USA}
\author{M. Jeong}
\affiliation{Dept. of Physics, Sungkyunkwan University, Suwon 16419, Korea}
\author{B. J. P. Jones}
\affiliation{Dept. of Physics, University of Texas at Arlington, 502 Yates St., Science Hall Rm 108, Box 19059, Arlington, TX 76019, USA}
\author{R. Joppe}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{D. Kang}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{W. Kang}
\affiliation{Dept. of Physics, Sungkyunkwan University, Suwon 16419, Korea}
\author{X. Kang}
\affiliation{Dept. of Physics, Drexel University, 3141 Chestnut Street, Philadelphia, PA 19104, USA}
\author{A. Kappes}
\affiliation{Institut f{\"u}r Kernphysik, Westf{\"a}lische Wilhelms-Universit{\"a}t M{\"u}nster, D-48149 M{\"u}nster, Germany}
\author{D. Kappesser}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{T. Karg}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{M. Karl}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{A. Karle}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{U. Katz}
\affiliation{Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, D-91058 Erlangen, Germany}
\author{M. Kauer}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{M. Kellermann}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{J. L. Kelley}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{A. Kheirandish}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\author{J. Kim}
\affiliation{Dept. of Physics, Sungkyunkwan University, Suwon 16419, Korea}
\author{K. Kin}
\affiliation{Dept. of Physics and Institute for Global Prominent Research, Chiba University, Chiba 263-8522, Japan}
\author{T. Kintscher}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{J. Kiryluk}
\affiliation{Dept. of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794-3800, USA}
\author{S. R. Klein}
\affiliation{Dept. of Physics, University of California, Berkeley, CA 94720, USA}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\author{R. Koirala}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{H. Kolanoski}
\affiliation{Institut f{\"u}r Physik, Humboldt-Universit{\"a}t zu Berlin, D-12489 Berlin, Germany}
\author{L. K{\"o}pke}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{C. Kopper}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{S. Kopper}
\affiliation{Dept. of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\author{D. J. Koskinen}
\affiliation{Niels Bohr Institute, University of Copenhagen, DK-2100 Copenhagen, Denmark}
\author{P. Koundal}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{M. Kovacevich}
\affiliation{Dept. of Physics, Drexel University, 3141 Chestnut Street, Philadelphia, PA 19104, USA}
\author{M. Kowalski}
\affiliation{Institut f{\"u}r Physik, Humboldt-Universit{\"a}t zu Berlin, D-12489 Berlin, Germany}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{K. Krings}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{G. Kr{\"u}ckl}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{N. Kurahashi}
\affiliation{Dept. of Physics, Drexel University, 3141 Chestnut Street, Philadelphia, PA 19104, USA}
\author{A. Kyriacou}
\affiliation{Department of Physics, University of Adelaide, Adelaide, 5005, Australia}
\author{C. Lagunas Gualda}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{J. L. Lanfranchi}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\author{M. J. Larson}
\affiliation{Dept. of Physics, University of Maryland, College Park, MD 20742, USA}
\author{F. Lauber}
\affiliation{Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany}
\author{J. P. Lazar}
\affiliation{Department of Physics and Laboratory for Particle Physics and Cosmology, Harvard University, Cambridge, MA 02138, USA}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{K. Leonard}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{A. Leszczy{\'n}ska}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{Y. Li}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\author{Q. R. Liu}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{E. Lohfink}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{C. J. Lozano Mariscal}
\affiliation{Institut f{\"u}r Kernphysik, Westf{\"a}lische Wilhelms-Universit{\"a}t M{\"u}nster, D-48149 M{\"u}nster, Germany}
\author{L. Lu}
\affiliation{Dept. of Physics and Institute for Global Prominent Research, Chiba University, Chiba 263-8522, Japan}
\author{F. Lucarelli}
\affiliation{D{\'e}partement de physique nucl{\'e}aire et corpusculaire, Universit{\'e} de Gen{\`e}ve, CH-1211 Gen{\`e}ve, Switzerland}
\author{A. Ludwig}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\affiliation{Department of Physics and Astronomy, UCLA, Los Angeles, CA 90095, USA}
\author{W. Luszczak}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{Y. Lyu}
\affiliation{Dept. of Physics, University of California, Berkeley, CA 94720, USA}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\author{W. Y. Ma}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{J. Madsen}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{K. B. M. Mahn}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{Y. Makino}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{P. Mallik}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{S. Mancina}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{I. C. Mari{\c{s}}}
\affiliation{Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium}
\author{R. Maruyama}
\affiliation{Dept. of Physics, Yale University, New Haven, CT 06520, USA}
\author{K. Mase}
\affiliation{Dept. of Physics and Institute for Global Prominent Research, Chiba University, Chiba 263-8522, Japan}
\author{F. McNally}
\affiliation{Department of Physics, Mercer University, Macon, GA 31207-0001, USA}
\author{K. Meagher}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{A. Medina}
\affiliation{Dept. of Physics and Center for Cosmology and Astro-Particle Physics, Ohio State University, Columbus, OH 43210, USA}
\author{M. Meier}
\affiliation{Dept. of Physics and Institute for Global Prominent Research, Chiba University, Chiba 263-8522, Japan}
\author{S. Meighen-Berger}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{J. Merz}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{J. Micallef}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{D. Mockler}
\affiliation{Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium}
\author{G. Moment{\'e}}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{T. Montaruli}
\affiliation{D{\'e}partement de physique nucl{\'e}aire et corpusculaire, Universit{\'e} de Gen{\`e}ve, CH-1211 Gen{\`e}ve, Switzerland}
\author{R. W. Moore}
\affiliation{Dept. of Physics, University of Alberta, Edmonton, Alberta, Canada T6G 2E1}
\author{R. Morse}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{M. Moulai}
\affiliation{Dept. of Physics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{R. Naab}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{R. Nagai}
\affiliation{Dept. of Physics and Institute for Global Prominent Research, Chiba University, Chiba 263-8522, Japan}
\author{U. Naumann}
\affiliation{Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany}
\author{J. Necker}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{L. V. Nguy{\~{\^{{e}}}}n}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{H. Niederhausen}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{M. U. Nisa}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{S. C. Nowicki}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{D. R. Nygren}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\author{A. Obertacke Pollmann}
\affiliation{Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany}
\author{M. Oehler}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{A. Olivas}
\affiliation{Dept. of Physics, University of Maryland, College Park, MD 20742, USA}
\author{E. O'Sullivan}
\affiliation{Dept. of Physics and Astronomy, Uppsala University, Box 516, S-75120 Uppsala, Sweden}
\author{H. Pandya}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{D. V. Pankova}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\author{N. Park}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{G. K. Parker}
\affiliation{Dept. of Physics, University of Texas at Arlington, 502 Yates St., Science Hall Rm 108, Box 19059, Arlington, TX 76019, USA}
\author{E. N. Paudel}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{P. Peiffer}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{C. P{\'e}rez de los Heros}
\affiliation{Dept. of Physics and Astronomy, Uppsala University, Box 516, S-75120 Uppsala, Sweden}
\author{S. Philippen}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{D. Pieloth}
\affiliation{Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany}
\author{S. Pieper}
\affiliation{Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany}
\author{A. Pizzuto}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{M. Plum}
\affiliation{Department of Physics, Marquette University, Milwaukee, WI, 53201, USA}
\author{Y. Popovych}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{A. Porcelli}
\affiliation{Dept. of Physics and Astronomy, University of Gent, B-9000 Gent, Belgium}
\author{M. Prado Rodriguez}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{P. B. Price}
\affiliation{Dept. of Physics, University of California, Berkeley, CA 94720, USA}
\author{B. Pries}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{G. T. Przybylski}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\author{C. Raab}
\affiliation{Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium}
\author{A. Raissi}
\affiliation{Dept. of Physics and Astronomy, University of Canterbury, Private Bag 4800, Christchurch, New Zealand}
\author{M. Rameez}
\affiliation{Niels Bohr Institute, University of Copenhagen, DK-2100 Copenhagen, Denmark}
\author{K. Rawlins}
\affiliation{Dept. of Physics and Astronomy, University of Alaska Anchorage, 3211 Providence Dr., Anchorage, AK 99508, USA}
\author{I. C. Rea}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{A. Rehman}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{R. Reimann}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{M. Renschler}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{G. Renzi}
\affiliation{Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium}
\author{E. Resconi}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{S. Reusch}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{W. Rhode}
\affiliation{Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany}
\author{M. Richman}
\affiliation{Dept. of Physics, Drexel University, 3141 Chestnut Street, Philadelphia, PA 19104, USA}
\author{B. Riedel}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{S. Robertson}
\affiliation{Dept. of Physics, University of California, Berkeley, CA 94720, USA}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\author{G. Roellinghoff}
\affiliation{Dept. of Physics, Sungkyunkwan University, Suwon 16419, Korea}
\author{M. Rongen}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{C. Rott}
\affiliation{Dept. of Physics, Sungkyunkwan University, Suwon 16419, Korea}
\author{T. Ruhe}
\affiliation{Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany}
\author{D. Ryckbosch}
\affiliation{Dept. of Physics and Astronomy, University of Gent, B-9000 Gent, Belgium}
\author{D. Rysewyk Cantu}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{I. Safa}
\affiliation{Department of Physics and Laboratory for Particle Physics and Cosmology, Harvard University, Cambridge, MA 02138, USA}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{S. E. Sanchez Herrera}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{A. Sandrock}
\affiliation{Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany}
\author{J. Sandroos}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{M. Santander}
\affiliation{Dept. of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\author{S. Sarkar}
\affiliation{Dept. of Physics, University of Oxford, Parks Road, Oxford OX1 3PU, UK}
\author{S. Sarkar}
\affiliation{Dept. of Physics, University of Alberta, Edmonton, Alberta, Canada T6G 2E1}
\author{K. Satalecka}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{M. Scharf}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{M. Schaufel}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{H. Schieler}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{P. Schlunder}
\affiliation{Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany}
\author{T. Schmidt}
\affiliation{Dept. of Physics, University of Maryland, College Park, MD 20742, USA}
\author{A. Schneider}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{J. Schneider}
\affiliation{Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, D-91058 Erlangen, Germany}
\author{F. G. Schr{\"o}der}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{L. Schumacher}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{S. Sclafani}
\affiliation{Dept. of Physics, Drexel University, 3141 Chestnut Street, Philadelphia, PA 19104, USA}
\author{D. Seckel}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{S. Seunarine}
\affiliation{Dept. of Physics, University of Wisconsin, River Falls, WI 54022, USA}
\author{S. Shefali}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{M. Silva}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{B. Smithers}
\affiliation{Dept. of Physics, University of Texas at Arlington, 502 Yates St., Science Hall Rm 108, Box 19059, Arlington, TX 76019, USA}
\author{R. Snihur}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{J. Soedingrekso}
\affiliation{Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany}
\author{D. Soldin}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{G. M. Spiczak}
\affiliation{Dept. of Physics, University of Wisconsin, River Falls, WI 54022, USA}
\author{C. Spiering}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\thanks{also at National Research Nuclear University, Moscow Engineering Physics Institute (MEPhI), Moscow 115409, Russia}
\author{J. Stachurska}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{M. Stamatikos}
\affiliation{Dept. of Physics and Center for Cosmology and Astro-Particle Physics, Ohio State University, Columbus, OH 43210, USA}
\author{T. Stanev}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{R. Stein}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{J. Stettner}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{A. Steuer}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{T. Stezelberger}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\author{R. G. Stokstad}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\author{T. Stuttard}
\affiliation{Niels Bohr Institute, University of Copenhagen, DK-2100 Copenhagen, Denmark}
\author{G. W. Sullivan}
\affiliation{Dept. of Physics, University of Maryland, College Park, MD 20742, USA}
\author{I. Taboada}
\affiliation{School of Physics and Center for Relativistic Astrophysics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\author{F. Tenholt}
\affiliation{Fakult{\"a}t f{\"u}r Physik {\&} Astronomie, Ruhr-Universit{\"a}t Bochum, D-44780 Bochum, Germany}
\author{S. Ter-Antonyan}
\affiliation{Dept. of Physics, Southern University, Baton Rouge, LA 70813, USA}
\author{S. Tilav}
\affiliation{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}
\author{F. Tischbein}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{K. Tollefson}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{L. Tomankova}
\affiliation{Fakult{\"a}t f{\"u}r Physik {\&} Astronomie, Ruhr-Universit{\"a}t Bochum, D-44780 Bochum, Germany}
\author{C. T{\"o}nnis}
\affiliation{Institute of Basic Science, Sungkyunkwan University, Suwon 16419, Korea}
\author{S. Toscano}
\affiliation{Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium}
\author{D. Tosi}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{A. Trettin}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{M. Tselengidou}
\affiliation{Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, D-91058 Erlangen, Germany}
\author{C. F. Tung}
\affiliation{School of Physics and Center for Relativistic Astrophysics, Georgia Institute of Technology, Atlanta, GA 30332, USA}
\author{A. Turcati}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{R. Turcotte}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{C. F. Turley}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\author{J. P. Twagirayezu}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{B. Ty}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{M. A. Unland Elorrieta}
\affiliation{Institut f{\"u}r Kernphysik, Westf{\"a}lische Wilhelms-Universit{\"a}t M{\"u}nster, D-48149 M{\"u}nster, Germany}
\author{J. Vandenbroucke}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{D. van Eijk}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{N. van Eijndhoven}
\affiliation{Vrije Universiteit Brussel (VUB), Dienst ELEM, B-1050 Brussels, Belgium}
\author{D. Vannerom}
\affiliation{Dept. of Physics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{J. van Santen}
\affiliation{DESY, D-15738 Zeuthen, Germany}
\author{S. Verpoest}
\affiliation{Dept. of Physics and Astronomy, University of Gent, B-9000 Gent, Belgium}
\author{M. Vraeghe}
\affiliation{Dept. of Physics and Astronomy, University of Gent, B-9000 Gent, Belgium}
\author{C. Walck}
\affiliation{Oskar Klein Centre and Dept. of Physics, Stockholm University, SE-10691 Stockholm, Sweden}
\author{A. Wallace}
\affiliation{Department of Physics, University of Adelaide, Adelaide, 5005, Australia}
\author{T. B. Watson}
\affiliation{Dept. of Physics, University of Texas at Arlington, 502 Yates St., Science Hall Rm 108, Box 19059, Arlington, TX 76019, USA}
\author{C. Weaver}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\author{A. Weindl}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{M. J. Weiss}
\affiliation{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\author{J. Weldert}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{C. Wendt}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{J. Werthebach}
\affiliation{Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany}
\author{M. Weyrauch}
\affiliation{Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany }
\author{B. J. Whelan}
\affiliation{Department of Physics, University of Adelaide, Adelaide, 5005, Australia}
\author{N. Whitehorn}
\affiliation{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}
\affiliation{Department of Physics and Astronomy, UCLA, Los Angeles, CA 90095, USA}
\author{K. Wiebe}
\affiliation{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}
\author{C. H. Wiebusch}
\affiliation{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}
\author{D. R. Williams}
\affiliation{Dept. of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\author{M. Wolf}
\affiliation{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}
\author{K. Woschnagg}
\affiliation{Dept. of Physics, University of California, Berkeley, CA 94720, USA}
\author{G. Wrede}
\affiliation{Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, D-91058 Erlangen, Germany}
\author{J. Wulff}
\affiliation{Fakult{\"a}t f{\"u}r Physik {\&} Astronomie, Ruhr-Universit{\"a}t Bochum, D-44780 Bochum, Germany}
\author{X. W. Xu}
\affiliation{Dept. of Physics, Southern University, Baton Rouge, LA 70813, USA}
\author{Y. Xu}
\affiliation{Dept. of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794-3800, USA}
\author{J. P. Yanez}
\affiliation{Dept. of Physics, University of Alberta, Edmonton, Alberta, Canada T6G 2E1}
\author{S. Yoshida}
\affiliation{Dept. of Physics and Institute for Global Prominent Research, Chiba University, Chiba 263-8522, Japan}
\author{T. Yuan}
\affiliation{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textendash}Madison, Madison, WI 53706, USA}
\author{Z. Zhang}
\affiliation{Dept. of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794-3800, USA}
\date{\today}

\collaboration{IceCube Collaboration}
\noaffiliation

==> A search for time-dependent neutrino emission with IceCube data from 2012 to 2017_v8/biblio.tex <==
@article{Aab:2017tyv,
      author         = "Aab, Alexander and others",
      title          = "{Observation of a Large-scale Anisotropy in the Arrival
      Directions of Cosmic Rays above $8 \times 10^{18}$ eV}",
      collaboration  = "Pierre Auger",
      journal        = "Science",
      volume         = "357",
      year           = "2017",
      number         = "6537",
      pages          = "1266-1270",
      doi            = "10.1126/science.aan4338",
      eprint         = "1709.07321",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      reportNumber   = "FERMILAB-PUB-17-354",
      SLACcitation   = "%%CITATION = ARXIV:1709.07321;%%"
}
@ARTICLE{2016ApJ...824L..20A,
       author = {{Ackermann}, M. and {Anantua}, R. and {Asano}, K. and {Baldini}, L. and
         {Barbiellini}, G. and {Bastieri}, D. and {Becerra Gonzalez}, J. and
         {Bellazzini}, R. and {Bissaldi}, E. and {Blandford}, R.~D. and
         {Bloom}, E.~D. and {Bonino}, R. and {Bottacini}, E. and {Bruel}, P. and
         {Buehler}, R. and {Caliandro}, G.~A. and {Cameron}, R.~A. and
         {Caragiulo}, M. and {Caraveo}, P.~A. and {Cavazzuti}, E. and
         {Cecchi}, C. and {Cheung}, C.~C. and {Chiang}, J. and {Chiaro}, G. and
         {Ciprini}, S. and {Cohen-Tanugi}, J. and {Costanza}, F. and
         {Cutini}, S. and {D'Ammando}, F. and {de Palma}, F. and {Desiante}, R. and
         {Digel}, S.~W. and {Di Lalla}, N. and {Di Mauro}, M. and
         {Di Venere}, L. and {Drell}, P.~S. and {Favuzzi}, C. and
         {Fegan}, S.~J. and {Ferrara}, E.~C. and {Fukazawa}, Y. and {Funk}, S. and
         {Fusco}, P. and {Gargano}, F. and {Gasparrini}, D. and {Giglietto}, N. and
         {Giordano}, F. and {Giroletti}, M. and {Grenier}, I.~A. and
         {Guillemot}, L. and {Guiriec}, S. and {Hayashida}, M. and {Hays}, E. and
         {Horan}, D. and {J{\'o}hannesson}, G. and {Kensei}, S. and
         {Kocevski}, D. and {Kuss}, M. and {La Mura}, G. and {Larsson}, S. and
         {Latronico}, L. and {Li}, J. and {Longo}, F. and {Loparco}, F. and
         {Lott}, B. and {Lovellette}, M.~N. and {Lubrano}, P. and
         {Madejski}, G.~M. and {Magill}, J.~D. and {Maldera}, S. and
         {Manfreda}, A. and {Mayer}, M. and {Mazziotta}, M.~N. and
         {Michelson}, P.~F. and {Mirabal}, N. and {Mizuno}, T. and
         {Monzani}, M.~E. and {Morselli}, A. and {Moskalenko}, I.~V. and
         {Nalewajko}, K. and {Negro}, M. and {Nuss}, E. and {Ohsugi}, T. and
         {Orlando}, E. and {Paneque}, D. and {Perkins}, J.~S. and
         {Pesce-Rollins}, M. and {Piron}, F. and {Pivato}, G. and
         {Porter}, T.~A. and {Principe}, G. and {Rando}, R. and {Razzano}, M. and
         {Razzaque}, S. and {Reimer}, A. and {Scargle}, J.~D. and
         {Sgr{\`o}}, C. and {Sikora}, M. and {Simone}, D. and {Siskind}, E.~J. and
         {Spada}, F. and {Spinelli}, P. and {Stawarz}, L. and {Thayer}, J.~B. and
         {Thompson}, D.~J. and {Torres}, D.~F. and {Troja}, E. and
         {Uchiyama}, Y. and {Yuan}, Y. and {Zimmer}, S.},
        title = "{Minute-timescale \&gt;100 MeV {\ensuremath{\gamma}}-Ray Variability during the Giant Outburst of Quasar 3C 279 Observed by Fermi-LAT in 2015 June}",
      journal = {\apjl},
     keywords = {galaxies: active, galaxies: jets, gamma rays: galaxies, quasars: individual: 3C 279, radiation mechanisms: non-thermal, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = jun,
       volume = {824},
       number = {2},
          eid = {L20},
        pages = {L20},
          doi = {10.3847/2041-8205/824/2/L20},
archivePrefix = {arXiv},
       eprint = {1605.05324},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...824L..20A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2015ApJ...807...79H,
       author = {{Hayashida}, M. and {Nalewajko}, K. and {Madejski}, G.~M. and
         {Sikora}, M. and {Itoh}, R. and {Ajello}, M. and {Blandford}, R.~D. and
         {Buson}, S. and {Chiang}, J. and {Fukazawa}, Y. and {Furniss}, A.~K. and
         {Urry}, C.~M. and {Hasan}, I. and {Harrison}, F.~A. and {Alexand
        er}, D.~M. and {Balokovi{\'c}}, M. and {Barret}, D. and {Boggs}, S.~E. and
         {Christensen}, F.~E. and {Craig}, W.~W. and {Forster}, K. and
         {Giommi}, P. and {Grefenstette}, B. and {Hailey}, C. and
         {Hornstrup}, A. and {Kitaguchi}, T. and {Koglin}, J.~E. and
         {Madsen}, K.~K. and {Mao}, P.~H. and {Miyasaka}, H. and {Mori}, K. and
         {Perri}, M. and {Pivovaroff}, M.~J. and {Puccetti}, S. and {Rana}, V. and
         {Stern}, D. and {Tagliaferri}, G. and {Westergaard}, N.~J. and
         {Zhang}, W.~W. and {Zoglauer}, A. and {Gurwell}, M.~A. and
         {Uemura}, M. and {Akitaya}, H. and {Kawabata}, K.~S. and
         {Kawaguchi}, K. and {Kanda}, Y. and {Moritani}, Y. and {Takaki}, K. and
         {Ui}, T. and {Yoshida}, M. and {Agarwal}, A. and {Gupta}, A.~C.},
        title = "{Rapid Variability of Blazar 3C 279 during Flaring States in 2013-2014 with Joint Fermi-LAT, NuSTAR, Swift, and Ground-Based Multiwavelength Observations}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: jets, gamma rays: galaxies, quasars: individual: 3C 279, radiation mechanisms: non-thermal, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = jul,
       volume = {807},
       number = {1},
          eid = {79},
        pages = {79},
          doi = {10.1088/0004-637X/807/1/79},
archivePrefix = {arXiv},
       eprint = {1502.04699},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...807...79H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Mannheim:1998wp,
      author         = "Mannheim, Karl and Protheroe, R. J. and Rachen, Jorg P.",
      title          = "{On the cosmic ray bound for models of extragalactic
                        neutrino production}",
      journal        = "Phys. Rev.",
      volume         = "D63",
      year           = "2001",
      pages          = "023003",
      doi            = "10.1103/PhysRevD.63.023003",
      eprint         = "astro-ph/9812398",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/9812398;%%"
}
@article{Waxman:1998yy,
      author         = "Waxman, Eli and Bahcall, John N.",
      title          = "{High-energy neutrinos from astrophysical sources: An
                        Upper bound}",
      journal        = "Phys. Rev.",
      volume         = "D59",
      year           = "1999",
      pages          = "023002",
      doi            = "10.1103/PhysRevD.59.023002",
      eprint         = "hep-ph/9807282",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IASSNS-AST-98-38",
      SLACcitation   = "%%CITATION = HEP-PH/9807282;%%"
}
@article{PhysRev.46.76.2,
  title = {Remarks on Super-Novae and Cosmic Rays},
  author = {Baade, W. and Zwicky, F.},
  journal = {Phys. Rev.},
  volume = {46},
  issue = {1},
  pages = {76--77},
  numpages = {0},
  year = {1934},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.46.76.2},
  url = {https://link.aps.org/doi/10.1103/PhysRev.46.76.2}
}
@ARTICLE{1984ARA&A..22..425H,
       author = {{Hillas}, A.~M.},
        title = "{The Origin of Ultra-High-Energy Cosmic Rays}",
      journal = {\araa},
         year = "1984",
        month = "Jan",
       volume = {22},
        pages = {425-444},
          doi = {10.1146/annurev.aa.22.090184.002233},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984ARA&A..22..425H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Gross:2010qma,
      author         = "Gross, Eilam and Vitells, Ofer",
      title          = "{Trial factors for the look elsewhere effect in high
                        energy physics}",
      journal        = "Eur. Phys. J.",
      volume         = "C70",
      year           = "2010",
      pages          = "525-530",
      doi            = "10.1140/epjc/s10052-010-1470-8",
      eprint         = "1005.1891",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.data-an",
      SLACcitation   = "%%CITATION = ARXIV:1005.1891;%%"
}

@article{aartsen2013first,
  title={First observation of PeV-energy neutrinos with IceCube},
  author={Aartsen, M.G. and others},
  journal={Physical review letters},
  volume={111},
  number={2},
  pages={021103},
  year={2013},
  publisher={APS}
}
@article{Aartsen:2013jdh,
      author         = "Aartsen, M. G. and others",
      title          = "{Evidence for High-Energy Extraterrestrial Neutrinos at
                        the IceCube Detector}",
      collaboration  = "IceCube",
      journal        = "Science",
      volume         = "342",
      year           = "2013",
      pages          = "1242856",
      doi            = "10.1126/science.1242856",
      eprint         = "1311.5238",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1311.5238;%%"
}
@article{BRAUN2010175,
title = "Time-dependent point source search methods in high energy neutrino astronomy",
journal = "Astroparticle Physics",
volume = "33",
number = "3",
pages = "175 - 181",
year = "2010",
issn = "0927-6505",
doi = "https://doi.org/10.1016/j.astropartphys.2010.01.005",
url = "http://www.sciencedirect.com/science/article/pii/S0927650510000241",
author = "Jim Braun and Mike Baker and Jon Dumm and Chad Finley and Albrecht Karle and Teresa Montaruli",
keywords = "Neutrino, Point source, Flare, Burst, Search method",
}
@article{Aartsen_2013,
	doi = {10.1088/0004-637x/779/2/132},
	year = {2013},
	month = {dec},
	publisher = {{IOP}, Publishing},
	volume = {779},
	number = {2},
	pages = {132},
	author = {Aartsen, M. G. and others},
	title = {Search for time-independent neutrino emission from astrophysical sources with 3 yr of IceCube data},
	journal = {The Astrophysical Journal}
}

@ARTICLE{2019arXiv191006006U,
       author = {Uro\v{s}evi\'c, Dejan and Arbutina, Bojan and
         Oni\'c, Du\v{s}an},
        title = "{Particle acceleration in interstellar shocks}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Oct",
          eid = {arXiv:1910.06006},
        pages = {arXiv:1910.06006},
archivePrefix = {arXiv},
       eprint = {1910.06006},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv191006006U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2012APh....35..660K,
       author = {{Kampert}, Karl-Heinz and {Unger}, Michael},
        title = "{Measurements of the cosmic ray composition with air shower experiments}",
      journal = {Astroparticle Physics},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = may,
       volume = {35},
       number = {10},
        pages = {660-678},
          doi = {10.1016/j.astropartphys.2012.02.004},
archivePrefix = {arXiv},
       eprint = {1201.0018},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012APh....35..660K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{Fermitools,
author = "{The Fermi Collaboration}",
title = "{Fermi Science Tools v9r31}",
note = "{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/documentation/}}"
}

@article{bell1978acceleration,
  title={The acceleration of cosmic rays in shock fronts--I},
  author={Bell, A.R.},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={182},
  number={2},
  pages={147--156},
  year={1978},
  publisher={Oxford University Press Oxford, UK}
}

@article{Aartsen:2016nxy,
      author         = "Aartsen, M. G. and others",
      title          = "{The IceCube Neutrino Observatory: Instrumentation and
                        Online Systems}",
      collaboration  = "IceCube",
      journal        = "JINST",
      volume         = "12",
      year           = "2017",
      number         = "03",
      pages          = "P03012",
      doi            = "10.1088/1748-0221/12/03/P03012",
      eprint         = "1612.05093",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      SLACcitation   = "%%CITATION = ARXIV:1612.05093;%%"
}

@article{Abbasi:2010vc,
    author = "Abbasi, R. and others",
    archivePrefix = "arXiv",
    collaboration = "IceCube",
    doi = "10.1016/j.nima.2010.03.102",
    eprint = "1002.2442",
    journal = "Nucl. Instrum. Meth. A",
    pages = "139--152",
    primaryClass = "astro-ph.IM",
    title = "{Calibration and Characterization of the IceCube Photomultiplier Tube}",
    volume = "618",
    year = "2010"
}

@article{Abbasi:2008aa,
      author         = "Abbasi, R. and others",
      title          = "{The IceCube Data Acquisition System: Signal Capture,
                        Digitization, and Timestamping}",
      collaboration  = "IceCube",
      journal        = "Nucl. Instrum. Meth.",
      volume         = "A601",
      year           = "2009",
      pages          = "294-316",
      doi            = "10.1016/j.nima.2009.01.001",
      eprint         = "0810.4930",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:0810.4930;%%"
}
@article{Schlickeiser,
author = {Schlickeiser, Reinhard},
year = {1988},
month = {12},
pages = {243-293},
title = {Cosmic-ray transport and acceleration. I - Derivation of the kinetic equation and application to cosmic rays in static cold media. II - Cosmic rays in moving cold media with application to diffusive shock wave acceleration},
volume = {336},
journal = {The Astrophysical Journal},
doi = {10.1086/167009}
}

@inproceedings{aller1987evidence,
  title={Evidence for shocks in relativistic jets},
  author={Aller, Hugh D and Hughes, Philip A and Aller, Margo F},
  booktitle={Superluminal Radio Sources},
  pages={273--279},
  editor={{Zensus}, J. Anton and {Pearson}, Timothy J.},
  year={1987}
}

@article{1990Ap&SS.171...13K,
       author = {{Kidger}, M.~R. and {Garcia Lario}, P. and {de Diego}, J.~A.},
        title = "{Visible and near-infrared monitoring of 3C 279 in 1988 1989}",
      journal = {Astrophysics \& Space Science (\apss)},
     keywords = {Astronomical Spectroscopy, Charge Coupled Devices, Galactic Structure, Light Curve, Near Infrared Radiation, Telescopes, Annual Variations, Stellar Luminosity, Visible Spectrum, Astrophysics},
         year = "1990",
        month = "Sep",
       volume = {171},
       number = {1-2},
        pages = {13-15},
          doi = {10.1007/BF00646813},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990Ap&SS.171...13K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2018arXiv181107979I,
       author = { {Aartsen}, M.~G. and others},
        title = "{Search for steady point-like sources in the astrophysical muon neutrino flux with 8 years of IceCube data}",
      journal = {arXiv e-prints},
     keywords = {High Energy Physics - Phenomenology, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2018",
        month = "Nov",
          eid = {arXiv:1811.07979},
        pages = {arXiv:1811.07979},
archivePrefix = {arXiv},
       eprint = {1811.07979},
 primaryClass = {hep-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv181107979I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{1989ApJ...347L...9M,
       author = {{Makino}, F. and {Kii}, T. and {Hayashida}, K. and {Inoue}, H. and
         {Tanaka}, Y. and {Ohashi}, T. and {Makishima}, K. and {Awaki}, H. and
         {Koyama}, K. and {Turner}, M.~J.~L. and {Williams}, O.~R.},
        title = "{X-Ray Outburst of the Quasar 3C 279}",
      journal = {\apjl},
     keywords = {Quasars, X Ray Sources, Astronomical Spectroscopy, Gravitational Effects, Hubble Constant, X Ray Spectra, Astrophysics, GALAXIES: JETS, QUASARS, X-RAYS: SOURCES, X-RAYS: SPECTRA},
         year = "1989",
        month = "Dec",
       volume = {347},
        pages = {L9},
          doi = {10.1086/185594},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1989ApJ...347L...9M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{PhysRevD.75.043006,
  title = {Calculation of atmospheric neutrino flux using the interaction model calibrated with atmospheric muon data},
  author = {Honda, M. and Kajita, T. and Kasahara, K. and Midorikawa, S. and Sanuki, T.},
  journal = {Phys. Rev. D},
  volume = {75},
  issue = {4},
  pages = {043006},
  numpages = {26},
  year = {2007},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.75.043006},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.75.043006}
}

@article{GAISSER2012801,
title = "Spectrum of cosmic-ray nucleons, kaon production, and the atmospheric muon charge ratio",
journal = "Astroparticle Physics",
volume = "35",
number = "12",
pages = "801 - 806",
year = "2012",
issn = "0927-6505",
doi = "https://doi.org/10.1016/j.astropartphys.2012.02.010",
url = "http://www.sciencedirect.com/science/article/pii/S0927650512000497",
author = "Thomas K. Gaisser",
keywords = "Cosmic rays, Muons, Neutrinos",
abstract = "Interpretation of measurements of the muon charge ratio in the TeV range depends on the spectra of protons and neutrons in the primary cosmic radiation and on the inclusive cross sections for production of π± and K± in the atmosphere. Recent measurements of the spectra of cosmic-ray nuclei are used here to estimate separately the energy spectra of protons and neutrons and hence to calculate the charge separated hadronic cascade in the atmosphere. From the corresponding production spectra of μ+ and μ− the μ+/μ− ratio is calculated and compared to recent measurements. The comparison leads to a determination of the relative contribution of kaons and pions. Implications for the spectra of νμ and ν¯μ are discussed."
}

@article{Aartsen:2013eka,
      author         = "Aartsen, M. G. and others",
      title          = "{Search for a diffuse flux of astrophysical muon
                        neutrinos with the IceCube 59-string configuration}",
      collaboration  = "IceCube",
      journal        = "Phys. Rev.",
      volume         = "D89",
      year           = "2014",
      number         = "6",
      pages          = "062007",
      doi            = "10.1103/PhysRevD.89.062007",
      eprint         = "1311.7048",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1311.7048;%%"
}

@article{IceCube:2018dnn,
      author         = "Aartsen, M. G. and others",
      title          = "{Multimessenger observations of a flaring blazar
                        coincident with high-energy neutrino IceCube-170922A}",
      collaboration  = "IceCube, Fermi-LAT, MAGIC, AGILE, ASAS-SN, HAWC,
                        H.E.S.S., INTEGRAL, Kanata, Kiso, Kapteyn, Liverpool
                        Telescope, Subaru, Swift NuSTAR, VERITAS, VLA/17B-403",
      journal        = "Science",
      volume         = "361",
      year           = "2018",
      number         = "6398",
      pages          = "eaat1378",
      doi            = "10.1126/science.aat1378",
      eprint         = "1807.08816",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1807.08816;%%"
}


@article{IceCube:2018cha,
      author         = "Aartsen, M. G. and others",
      title          = "{Neutrino emission from the direction of the blazar TXS
                        0506+056 prior to the IceCube-170922A alert}",
      collaboration  = "IceCube",
      journal        = "Science",
      volume         = "361",
      year           = "2018",
      number         = "6398",
      pages          = "147-151",
      doi            = "10.1126/science.aat2890",
      eprint         = "1807.08794",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1807.08794;%%"
}
@article{Aartsen:2015wto,
      author         = "Aartsen, M. G. and others",
      title          = "{Searches for Time Dependent Neutrino Sources with
                        IceCube Data from 2008 to 2012}",
      collaboration  = "IceCube",
      journal        = "Astrophys. J.",
      volume         = "807",
      year           = "2015",
      number         = "1",
      pages          = "46",
      doi            = "10.1088/0004-637X/807/1/46",
      eprint         = "1503.00598",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1503.00598;%%"
}
@article{aartsen2015atmospheric,
  title={Atmospheric and astrophysical neutrinos above 1 TeV interacting in IceCube},
  author={Aartsen, M. G. and others},
  journal={Physical Review D},
  volume={91},
  number={2},
  pages={022001},
  year={2015},
  publisher={APS}
}
@article{aartsen2017icecube,
  title={The IceCube realtime alert system},
  author={Aartsen, M. G. and others},
  journal={Astroparticle Physics},
  volume={92},
  pages={30--41},
  year={2017},
  publisher={Elsevier}
}
https://www.overleaf.com/project/5c40b5044e3521578a21a88d
@article{aartsen2014searches,
  title={Searches for extended and point-like neutrino sources with four years of IceCube data},
  author={Aartsen, M. G. and others},
  journal={The Astrophysical Journal},
  volume={796},
  number={2},
  pages={109},
  year={2014},
  publisher={IOP Publishing}
}
@article{braun2008methods,
  title={Methods for point source analysis in high energy neutrino telescopes},
  author={Braun, Jim and Dumm, Jon and De Palma, Francesco and Finley, Chad and Karle, Albrecht and Montaruli, Teresa},
  journal={Astroparticle Physics},
  volume={29},
  number={4},
  pages={299--305},
  year={2008},
  publisher={Elsevier}
}
@article{braun2010time,
  title={Time-dependent point source search methods in high energy neutrino astronomy},
  author={Braun, Jim and Baker, Mike and Dumm, Jon and Finley, Chad and Karle, Albrecht and Montaruli, Teresa},
  journal={Astroparticle Physics},
  volume={33},
  number={3},
  pages={175--181},
  year={2010},
  publisher={Elsevier}
}

@ARTICLE{aartsen2017all,
       author = {{Aartsen}, M.~G. and others},
        title = "{All-sky Search for Time-integrated Neutrino Emission from Astrophysical Sources with 7 yr of IceCube Data}",
      journal = {\apj},
     keywords = {astroparticle physics, galaxies: active, neutrinos, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2017",
        month = "Feb",
       volume = {835},
       number = {2},
          eid = {151},
        pages = {151},
          doi = {10.3847/1538-4357/835/2/151},
archivePrefix = {arXiv},
       eprint = {1609.04981},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...835..151A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Abbasi_2011,
	doi = {10.1088/0004-637x/732/1/18},
	year = 2011,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {732},
	number = {1},
	pages = {18},
	author = {Abbasi, R. and others},
	title = {{TIME}-{INTEGRATED} {SEARCHES} {FOR} {POINT}-{LIKE} {SOURCES} {OF} {NEUTRINOS} {WITH} {THE} 40-{STRING} {IceCube} {DETECTOR}},
	journal = {The Astrophysical Journal}
}

@article{abbasi2011time,
  title={Time-dependent searches for point sources of neutrinos with the 40-string and 22-string configurations of IceCube},
  author={Abbasi, R. and others},
  journal={The Astrophysical Journal},
  volume={744},
  number={1},
  pages={1},
  year={2011},
  publisher={IOP Publishing}
}
@article{hartman1992detection,
  title={Detection of high-energy gamma radiation from quasar 3C 279 by the EGRET telescope on the Compton Gamma Ray Observatory},
  author={Hartman, RC and Bertsch, DL and Fichtel, CE and Hunter, SD and Kanbach, G and Kniffen, DA and Kwok, PW and Lin, YC and Mattox, JR and Mayer-Hasselwander, HA and others},
  journal={The Astrophysical Journal},
  volume={385},
  pages={L1--L4},
  year={1992}
}
@article{maraschi1992jet,
  title={A jet model for the gamma-ray emitting blazar 3C 279},
  author={Maraschi, L and Ghisellini, G and Celotti, A},
  journal={The Astrophysical Journal},
  volume={397},
  pages={L5--L9},
  year={1992}
}
@article{wehrle1998multiwavelength,
  title={Multiwavelength observations of a dramatic high-energy flare in the blazar 3C 279},
  author={Wehrle, Ann E and Pian, E and Urry, CM and Maraschi, L and McHardy, IM and Lawson, AJ and Ghisellini, G and Hartman, RC and Madejski, GM and Makino, F and others},
  journal={The Astrophysical Journal},
  volume={497},
  number={1},
  pages={178},
  year={1998},
  publisher={IOP Publishing}
}

@article{gammarays3C279MAGIC2009,
      author         = "Errando, M. and others",
      title          = "{Discovery of very high energy gamma-rays from the flat
                        spectrum radio quasar 3C 279 with the MAGIC telescope}",
      booktitle      = "{Proceedings, 4th Heidelberg International Symposium on
                        High-Energy Gamma Ray Astronomy: Heidelberg, Germany, July
                        7-11, 2008}",
      collaboration  = "MAGIC",
      journal        = "AIP Conf. Proc.",
      volume         = "1085",
      year           = "2009",
      number         = "1",
      pages          = "423-426",
      doi            = "10.1063/1.3076698",
      eprint         = "0901.3275",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:0901.3275;%%"
}

@article{Diltz_2015,
	doi = {10.1088/0004-637x/802/2/133},
	url = {https://doi.org/10.1088%2F0004-637x%2F802%2F2%2F133},
	year = 2015,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {802},
	number = {2},
	pages = {133},
	author = {C. Diltz and M. Böttcher and G. Fossati},
	title = {{TIME} {DEPENDENT} {HADRONIC} {MODELING} {OF} {FLAT} {SPECTRUM} {RADIO} {QUASARS}},
	journal = {The Astrophysical Journal},
}

@article{teshima2007discovery,
      author         = "Teshima, Masahiro and others",
      title          = "{Discovery of Very High Energy Gamma-Rays from the
                        Distant Flat Spectrum Radio Quasar 3C 279 with the MAGIC
                        Telescope}",
      collaboration  = "MAGIC",
      volume         = "3",
      year           = "2007",
      pages          = "1045",
      eprint         = "0709.1475",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "MPP-2007-111",
      SLACcitation   = "%%CITATION = ARXIV:0709.1475;%%"
}

@inproceedings{turler2012multiple,
  title={Multiple synchrotron self-Compton modeling of gamma-ray flares in 3C 279},
  author={T{\"u}rler, Marc and Bj{\"o}rnsson, Claes-Ingvar},
  booktitle={Journal of Physics: Conference Series},
  volume={355},
  number={1},
  pages={012033},
  year={2012},
  organization={IOP Publishing}
}

@article{paliya2016lepto,
  title={Lepto-Hadronic Origin of $\gamma$-ray Outbursts of 3C 279},
  author={Paliya, Vaidehi S and Diltz, Chris and Bottcher, Markus and Stalin, CS and Buckley, David},
  journal={arXiv preprint arXiv:1603.05506},
  year={2016}
}

@article{ackermann2016minute,
      author         = "Ackermann, M. and others",
      title          = "{Minute-Timescale >100 MeV gamma-ray variability during
                        the giant outburst of quasar 3C 279 observed by Fermi-LAT
                        in 2015 June}",
      collaboration  = "Fermi-LAT",
      journal        = "Astrophys. J.",
      volume         = "824",
      year           = "2016",
      number         = "2",
      pages          = "L20",
      doi            = "10.3847/2041-8205/824/2/L20",
      eprint         = "1605.05324",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1605.05324;%%"
}

@article{Aartsen:2019fau,
      author         = "Aartsen, M. G. and others",
      title          = "{Time-integrated Neutrino Source Searches with 10 years of IceCube Data}",
      collaboration  = "IceCube",
      year           = "2019",
      eprint         = "1910.08488",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1910.08488;%%"
}
@article{Ghisellini:2012hs,
      author         = "Ghisellini, Gabriele",
      title          = "{Radiative Processes in High Energy Astrophysics}",
      journal        = "Lect. Notes Phys.",
      volume         = "873",
      year           = "2013",
      pages          = "1-147",
      doi            = "10.1007/978-3-319-00612-3",
      eprint         = "1202.5949",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1202.5949;%%"
}
@INPROCEEDINGS{2019ICRC...36..209C,
       author = {{Caprioli}, D. and {Haggerty}, C.},
        title = "{The Issue with Diffusive Shock Acceleration}",
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Physics - Plasma Physics, Physics - Space Physics},
    booktitle = {36th International Cosmic Ray Conference (ICRC2019)},
         year = "2019",
       series = {International Cosmic Ray Conference},
       volume = {36},
        month = "Jul",
          eid = {209},
        pages = {209},
archivePrefix = {arXiv},
       eprint = {1909.06288},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ICRC...36..209C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Blandford:1987pw,
      author         = "Blandford, R. and Eichler, D.",
      title          = "{Particle Acceleration at Astrophysical Shocks: A Theory
                        of Cosmic Ray Origin}",
      journal        = "Phys. Rept.",
      volume         = "154",
      year           = "1987",
      pages          = "1-75",
      doi            = "10.1016/0370-1573(87)90134-7",
      SLACcitation   = "%%CITATION = PRPLC,154,1;%%"
}
@ARTICLE{2015ATel76331C,
   author = {{Cutini}, S.},
    title = "{Fermi LAT detection of renewed and strong GeV activity from blazar 3C 279}",
  journal = {The Astronomer's Telegram},
 keywords = {Request for Observations, AGN, Blazar, Quasar},
     year = 2015,
    month = jun,
   volume = 7633,
   adsurl = {http://adsabs.harvard.edu/abs/2015ATel.7633....1C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{scargle2013studies,
  title={Studies in astronomical time series analysis. VI. Bayesian block representations},
  author={Scargle, Jeffrey D and Norris, Jay P and Jackson, Brad and Chiang, James},
  journal={The Astrophysical Journal},
  volume={764},
  number={2},
  pages={167},
  year={2013},
  publisher={IOP Publishing}
}
@article{resconi2009classification,
  title={The classification of flaring states of blazars},
  author={Resconi, E and Franco, D and Gross, A and Costamante, L and Flaccomio, E},
  journal={Astronomy \& Astrophysics},
  volume={502},
  number={2},
  pages={499--504},
  year={2009},
  publisher={EDP Sciences}
}
@article{halzen2016high,
  title={High-energy Neutrinos from Recent Blazar Flares},
  author={Halzen, Francis and Kheirandish, Ali},
  journal={The Astrophysical Journal},
  volume={831},
  number={1},
  pages={12},
  year={2016},
  publisher={IOP Publishing}
}

@article{Neunhoffer:2004ha,
      author         = "Neunhoffer, Till",
      title          = "{Estimating the angular resolution of tracks in neutrino
                        telescopes based on a likelihood analysis}",
      journal        = "Astropart. Phys.",
      volume         = "25",
      year           = "2006",
      pages          = "220-225",
      doi            = "10.1016/j.astropartphys.2006.01.002",
      eprint         = "astro-ph/0403367",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0403367;%%"
}

@article{Halzen:2005pz,
      author         = "Halzen, Francis and Hooper, Dan",
      title          = "{High energy neutrinos from the TeV blazar 1ES 1959+650}",
      journal        = "Astropart. Phys.",
      volume         = "23",
      year           = "2005",
      pages          = "537-542",
      doi            = "10.1016/j.astropartphys.2005.03.007",
      eprint         = "astro-ph/0502449",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "MADPH-05-1415",
      SLACcitation   = "%%CITATION = ASTRO-PH/0502449;%%"
}

@article{Atwood:2013rka,
author = {Atwood, W. and Albert, A. and Baldini, L. and Tinivella, Marco and Bregeon, J. and Pesce Rollins, Melissa and Sgrò, C. and Bruel, P. and Charles, E. and Drlica-Wagner, A. and Franckowiak, Anna and Jogler, T. and Rochester, L. and Usher, T. and Wood, M. and Cohen‐Tanugi, Johann and Zimmer, Stephan},
year = {2013},
month = {03},
pages = {},
title = {Pass 8: Toward the Full Realization of the Fermi-LAT Scientific Potential}
}

@article{Aartsen_2016,
	doi = {10.3847/2041-8205/824/2/l28},
	url = {https://doi.org/10.3847%2F2041-8205%2F824%2F2%2Fl28},
	year = 2016,
	month = {jun},
	publisher = {American Astronomical Society},
	volume = {824},
	number = {2},
	pages = {L28},
	author = {M. G. Aartsen and K. Abraham and M. Ackermann and J. Adams and J. A. Aguilar and M. Ahlers and M. Ahrens and D. Altmann and K. Andeen and T. Anderson and I. Ansseau and G. Anton and M. Archinger and C. Arguelles and T. C. Arlen and J. Auffenberg and X. Bai and S. W. Barwick and V. Baum and R. Bay and J. J. Beatty and J. Becker Tjus and K.-H. Becker and S. BenZvi and P. Berghaus and D. Berley and E. Bernardini and A. Bernhard and D. Z. Besson and G. Binder and D. Bindig and M. Bissok and E. Blaufuss and S. Blot and D. J. Boersma and C. Bohm and M. Börner and F. Bos and D. Bose and S. Böser and O. Botner and J. Braun and L. Brayeur and H.-P. Bretz and A. Burgman and N. Buzinsky and J. Casey and M. Casier and E. Cheung and D. Chirkin and A. Christov and K. Clark and L. Classen and S. Coenders and G. H. Collin and J. M. Conrad and D. F. Cowen and A. H. Cruz Silva and J. Daughhetee and J. C. Davis and M. Day and J. P. A. M. de Andr{\'{e}} and C. De Clercq and E. del Pino Rosendo and H. Dembinski and S. De Ridder and P. Desiati and K. D. de Vries and G. de Wasseige and M. de With and T. DeYoung and J. C. D{\'{\i}}az-V{\'{e}}lez and V. di Lorenzo and H. Dujmovic and J. P. Dumm and M. Dunkman and B. Eberhardt and T. Ehrhardt and B. Eichmann and S. Euler and P. A. Evenson and S. Fahey and A. R. Fazely and J. Feintzeig and J. Felde and K. Filimonov and C. Finley and S. Flis and C.-C. Fösig and T. Fuchs and T. K. Gaisser and R. Gaior and J. Gallagher and L. Gerhardt and K. Ghorbani and L. Gladstone and M. Glagla and T. Glüsenkamp and A. Goldschmidt and G. Golup and J. G. Gonzalez and D. G{\'{o}}ra and D. Grant and Z. Griffith and C. Ha and C. Haack and A. Haj Ismail and A. Hallgren and F. Halzen and E. Hansen and B. Hansmann and T. Hansmann and K. Hanson and D. Hebecker and D. Heereman and K. Helbing and R. Hellauer and S. Hickford and J. Hignight and G. C. Hill and K. D. Hoffman and R. Hoffmann and K. Holzapfel and A. Homeier and K. Hoshina and F. Huang and M. Huber and W. Huelsnitz and K. Hultqvist and S. In and A. Ishihara and E. Jacobi and G. S. Japaridze and M. Jeong and K. Jero and B. J. P. Jones and M. Jurkovic and A. Kappes and T. Karg and A. Karle and U. Katz and M. Kauer and A. Keivani and J. L. Kelley and J. Kemp and A. Kheirandish and M. Kim and T. Kintscher and J. Kiryluk and S. R. Klein and G. Kohnen and R. Koirala and H. Kolanoski and R. Konietz and L. Köpke and C. Kopper and S. Kopper and D. J. Koskinen and M. Kowalski and K. Krings and M. Kroll and G. Krückl and C. Krüger and J. Kunnen and S. Kunwar and N. Kurahashi and T. Kuwabara and M. Labare and J. L. Lanfranchi and M. J. Larson and D. Lennarz and M. Lesiak-Bzdak and M. Leuermann and J. Leuner and L. Lu and J. Lünemann and J. Madsen and G. Maggi and K. B. M. Mahn and S. Mancina and M. Mandelartz and R. Maruyama and K. Mase and H. S. Matis and R. Maunu and F. McNally and K. Meagher and M. Medici and M. Meier and A. Meli and T. Menne and G. Merino and T. Meures and S. Miarecki and E. Middell and L. Mohrmann and T. Montaruli and R. Nahnhauer and U. Naumann and G. Neer and H. Niederhausen and S. C. Nowicki and D. R. Nygren and A. Obertacke Pollmann and A. Olivas and A. Omairat and A. O'Murchadha and T. Palczewski and H. Pandya and D. V. Pankova and Ö. Penek and J. A. Pepper and C. P{\'{e}}rez de los Heros and C. Pfendner and D. Pieloth and E. Pinat and J. Posselt and P. B. Price and G. T. Przybylski and M. Quinnan and C. Raab and L. Rädel and M. Rameez and K. Rawlins and R. Reimann and M. Relich and E. Resconi and W. Rhode and M. Richman and B. Riedel and S. Robertson and M. Rongen and C. Rott and T. Ruhe and D. Ryckbosch and L. Sabbatini and A. Sandrock and J. Sandroos and S. Sarkar and K. Satalecka and M. Schimp and P. Schlunder and T. Schmidt and S. Schoenen and S. Schöneberg and A. Schönwald and L. Schumacher and D. Seckel and S. Seunarine and D. Soldin and M. Song and G. M. Spiczak and C. Spiering and M. Stahlberg and M. Stamatikos and T. Stanev and A. Stasik and A. Steuer and T. Stezelberger and R. G. Stokstad and A. Stö{\ss}l and R. Ström and N. L. Strotjohann and G. W. Sullivan and M. Sutherland and H. Taavola and I. Taboada and J. Tatar and S. Ter-Antonyan and A. Terliuk and G. Te{\v{s}}i{\'{c}} and S. Tilav and P. A. Toale and M. N. Tobin and S. Toscano and D. Tosi and M. Tselengidou and A. Turcati and E. Unger and M. Usner and S. Vallecorsa and J. Vandenbroucke and N. van Eijndhoven and S. Vanheule and M. van Rossem and J. van Santen and J. Veenkamp and M. Vehring and M. Voge and M. Vraeghe and C. Walck and A. Wallace and M. Wallraff and N. Wandkowsky and Ch. Weaver and C. Wendt and S. Westerhoff and B. J. Whelan and N. Whitehorn and S. Wickmann and K. Wiebe and C. H. Wiebusch and L. Wille and D. R. Williams and L. Wills and H. Wissing and M. Wolf and T. R. Wood and K. Woschnagg and D. L. Xu and X. W. Xu and Y. Xu and J. P. Yanez and G. Yodh and S. Yoshida and M. Zoll and},
	title = {{LOWERING} {ICECUBE}{\textquotesingle}S {ENERGY} {THRESHOLD} {FOR} {POINT} {SOURCE} {SEARCHES} {IN} {THE} {SOUTHERN} {SKY}},
	journal = {The Astrophysical Journal},
	abstract = {Observation of a point source of astrophysical neutrinos would be a “smoking gun” signature of a cosmic-ray accelerator. While IceCube has recently discovered a diffuse flux of astrophysical neutrinos, no localized point source has been observed. Previous IceCube searches for point sources in the southern sky were restricted by either an energy threshold above a few hundred  TeV or poor neutrino angular resolution. Here we present a search for southern sky point sources with greatly improved sensitivities to neutrinos with energies below 100 TeV. By selecting charged-current ν

μ
 interacting inside the detector, we reduce the atmospheric background while retaining efficiency for astrophysical neutrino-induced events reconstructed with sub-degree angular resolution. The new event sample covers three years of detector data and leads to a factor of 10 improvement in sensitivity to point sources emitting below 100 TeV in the southern sky. No statistically significant evidence of point sources was found, and upper limits are set on neutrino emission from individual sources. A posteriori analysis of the highest-energy (∼100 TeV) starting event in the sample found that this event alone represents a 2.8σ deviation from the hypothesis that the data consists only of atmospheric background.}
}

@article{Sikora_2009,
	doi = {10.1088/0004-637x/704/1/38},
	url = {https://doi.org/10.1088%2F0004-637x%2F704%2F1%2F38},
	year = 2009,
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {704},
	number = {1},
	pages = {38--50},
	author = {Marek Sikora and {\L}ukasz Stawarz and Rafa{\l} Moderski and Krzysztof Nalewajko and Greg M. Madejski},
	title = {{CONSTRAINING} {EMISSION} {MODELS} {OF} {LUMINOUS} {BLAZAR} {SOURCES}},
	journal = {The Astrophysical Journal},
	abstract = {Many luminous blazars which are associated with quasar-type active galactic nuclei display broadband spectra characterized by a large luminosity ratio of their high-energy (γ-ray) and low-energy (synchrotron) spectral components. This large ratio, reaching values up to 100, challenges the standard synchrotron self-Compton models by means of substantial departures from the minimum power condition. Luminous blazars also typically have very hard X-ray spectra, and those in turn seem to challenge hadronic scenarios for the high-energy blazar emission. As shown in this paper, no such problems are faced by the models which involve Comptonization of radiation provided by a broad-line region, or dusty molecular torus. The lack or weakness of bulk-Compton and Klein-Nishina features indicated by the presently available data favors the production of γ-rays via upscattering of infrared photons from hot dust. This implies that the blazar emission zone is located at parsec-scale distances from the nucleus, and as such is possibly associated with the extended, quasi-stationary reconfinement shocks formed in relativistic outflows. This scenario predicts characteristic timescales for flux changes in luminous blazars to be days/weeks, consistent with the variability patterns observed in such systems at infrared, optical, and γ-ray frequencies. We also propose that the parsec-scale blazar activity can be occasionally accompanied by dissipative events taking place at sub-parsec distances and powered by internal shocks and/or reconnection of magnetic fields. These could account for the multiwavelength intraday flares occasionally observed in powerful blazar sources.}
}

@article{Abeysekara_2018,
	doi = {10.3847/2041-8213/aad053},
	url = {https://doi.org/10.3847%2F2041-8213%2Faad053},
	year = 2018,
	month = {jul},
	publisher = {American Astronomical Society},
	volume = {861},
	number = {2},
	pages = {L20},
	author = {A. U. Abeysekara and A. Archer and W. Benbow and R. Bird and A. Brill and R. Brose and J. H. Buckley and J. L. Christiansen and A. J. Chromey and M. K. Daniel and A. Falcone and Q. Feng and J. P. Finley and L. Fortson and A. Furniss and G. H. Gillanders and O. Gueta and D. Hanna and O. Hervet and J. Holder and G. Hughes and T. B. Humensky and C. A. Johnson and P. Kaaret and P. Kar and N. Kelley-Hoskins and M. Kertzman and D. Kieda and M. Krause and F. Krennrich and M. J. Lang and P. Moriarty and R. Mukherjee and S. O'Brien and R. A. Ong and A. N. Otte and N. Park and A. Petrashyk and M. Pohl and E. Pueschel and J. Quinn and K. Ragan and P. T. Reynolds and G. T. Richards and E. Roache and C. Rulten and I. Sadeh and M. Santander and S. S. Scott and G. H. Sembroski and K. Shahinyan and J. Tyler and S. P. Wakely and A. Weinstein and R. M. Wells and P. Wilcox and A. Wilhelm and D. A. Williams and T. J Williamson and B. Zitzer and A. Kaur and},
	title = {{VERITAS} Observations of the {BL} Lac Object {TXS} 0506$\mathplus$056},
	journal = {The Astrophysical Journal},
	abstract = {On 2017 September 22, the IceCube Neutrino Observatory reported the detection of the high-energy neutrino event IC 170922A, of potential astrophysical origin. It was soon determined that the neutrino direction was consistent with the location of the gamma-ray blazar TXS 0506+056 (3FGL J0509.4+0541), which was in an elevated gamma-ray emission state as measured by the Fermi satellite. Very Energetic Radiation Imaging Telescope Array System (VERITAS) observations of the neutrino/blazar region started on 2017 September 23 in response to the neutrino alert and continued through 2018 February 6. While no significant very-high-energy (VHE; E > 100 GeV) emission was observed from the blazar by VERITAS in the two-week period immediately following the IceCube alert, TXS 0506+056 was detected by VERITAS with a significance of 5.8 standard deviations (σ) in the full 35 hr data set. The average photon flux of the source during this period was (8.9 ± 1.6) × 10−12 cm−2 s−1, or 1.6% of the Crab Nebula flux, above an energy threshold of 110 GeV, with a soft spectral index of 4.8 ± 1.3.}
}

@article{Oikonomou_2019,
   title={High-energy neutrino flux from individual blazar flares},
   volume={489},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/stz2246},
   DOI={10.1093/mnras/stz2246},
   number={3},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Oikonomou, Foteini and Murase, Kohta and Padovani, Paolo and Resconi, Elisa and Meszaros, Peter},
   year={2019},
   month={Sep},
   pages={4347--4366}
}

@article{Penacchioni_2019,
	doi = {10.3847/2041-8213/ab0087},
	url = {https://doi.org/10.3847%2F2041-8213%2Fab0087},
	year = 2019,
	month = {jan},
	publisher = {American Astronomical Society},
	volume = {871},
	number = {2},
	pages = {L30},
	author = {A. V. Penacchioni and O. Civitarese},
	title = {Time Delay between Neutrinos and Gamma-Rays in Short Gamma-Ray Bursts},
	journal = {The Astrophysical Journal},
	abstract = {In this Letter we make an estimate of the time delay between signals, recorded at detectors on Earth, of neutrinos and photons originated in a short gamma-ray burst. We describe the geometry and dynamics of the system according to the Fireshell model. The delay in the photon’s arrival time is produced because the system is originally opaque to radiation; thus, the photons remain trapped and thermalize until the transparency condition is reached. We calculate the time interval between neutrino emission and photon emission in the black hole frame and transform it to the observer frame using Lorentz transformations. We obtain a difference in the arrival time at Earth of .}
}

@phdthesis{Christov:2016zti,
    author = "Christov, Asen",
    title = "{Multi-Messenger studies with the IceCube Detector}",
    doi = "10.13097/archive-ouverte/unige:91766",
    school = "Geneva U.",
    year = "2016"
}

@article{energyRecoMethods2014,
author = {Aartsen, M. and Ackermann, M. and Adams, J. and Aguilar Sánchez, Juan Antonio and Ahlers, M. and Altmann, David and Arguelles, C. and Auffenberg, J. and Bai, Xiaoqiong and Baker, Moatasem and Barwick, S. and Baum, V. and Bay, Ryan and Beatty, J. and Tjus, J. and Becker, K. and BenZvi, S. and Berghaus, P.},
year = {2014},
month = {03},
pages = {P03009},
title = {Energy Reconstruction Methods in the IceCube Neutrino Telescope},
volume = {9},
journal = {Journal of Instrumentation},
doi = {10.1088/1748-0221/9/03/P03009}
}

==> biblio.tex <==
@article{Aab:2017tyv,
      author         = "Aab, Alexander and others",
      title          = "{Observation of a Large-scale Anisotropy in the Arrival
      Directions of Cosmic Rays above $8 \times 10^{18}$ eV}",
      collaboration  = "Pierre Auger",
      journal        = "Science",
      volume         = "357",
      year           = "2017",
      number         = "6537",
      pages          = "1266-1270",
      doi            = "10.1126/science.aan4338",
      eprint         = "1709.07321",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      reportNumber   = "FERMILAB-PUB-17-354",
      SLACcitation   = "%%CITATION = ARXIV:1709.07321;%%"
}
@ARTICLE{2016ApJ...824L..20A,
       author = {{Ackermann}, M. and {Anantua}, R. and {Asano}, K. and {Baldini}, L. and
         {Barbiellini}, G. and {Bastieri}, D. and {Becerra Gonzalez}, J. and
         {Bellazzini}, R. and {Bissaldi}, E. and {Blandford}, R.~D. and
         {Bloom}, E.~D. and {Bonino}, R. and {Bottacini}, E. and {Bruel}, P. and
         {Buehler}, R. and {Caliandro}, G.~A. and {Cameron}, R.~A. and
         {Caragiulo}, M. and {Caraveo}, P.~A. and {Cavazzuti}, E. and
         {Cecchi}, C. and {Cheung}, C.~C. and {Chiang}, J. and {Chiaro}, G. and
         {Ciprini}, S. and {Cohen-Tanugi}, J. and {Costanza}, F. and
         {Cutini}, S. and {D'Ammando}, F. and {de Palma}, F. and {Desiante}, R. and
         {Digel}, S.~W. and {Di Lalla}, N. and {Di Mauro}, M. and
         {Di Venere}, L. and {Drell}, P.~S. and {Favuzzi}, C. and
         {Fegan}, S.~J. and {Ferrara}, E.~C. and {Fukazawa}, Y. and {Funk}, S. and
         {Fusco}, P. and {Gargano}, F. and {Gasparrini}, D. and {Giglietto}, N. and
         {Giordano}, F. and {Giroletti}, M. and {Grenier}, I.~A. and
         {Guillemot}, L. and {Guiriec}, S. and {Hayashida}, M. and {Hays}, E. and
         {Horan}, D. and {J{\'o}hannesson}, G. and {Kensei}, S. and
         {Kocevski}, D. and {Kuss}, M. and {La Mura}, G. and {Larsson}, S. and
         {Latronico}, L. and {Li}, J. and {Longo}, F. and {Loparco}, F. and
         {Lott}, B. and {Lovellette}, M.~N. and {Lubrano}, P. and
         {Madejski}, G.~M. and {Magill}, J.~D. and {Maldera}, S. and
         {Manfreda}, A. and {Mayer}, M. and {Mazziotta}, M.~N. and
         {Michelson}, P.~F. and {Mirabal}, N. and {Mizuno}, T. and
         {Monzani}, M.~E. and {Morselli}, A. and {Moskalenko}, I.~V. and
         {Nalewajko}, K. and {Negro}, M. and {Nuss}, E. and {Ohsugi}, T. and
         {Orlando}, E. and {Paneque}, D. and {Perkins}, J.~S. and
         {Pesce-Rollins}, M. and {Piron}, F. and {Pivato}, G. and
         {Porter}, T.~A. and {Principe}, G. and {Rando}, R. and {Razzano}, M. and
         {Razzaque}, S. and {Reimer}, A. and {Scargle}, J.~D. and
         {Sgr{\`o}}, C. and {Sikora}, M. and {Simone}, D. and {Siskind}, E.~J. and
         {Spada}, F. and {Spinelli}, P. and {Stawarz}, L. and {Thayer}, J.~B. and
         {Thompson}, D.~J. and {Torres}, D.~F. and {Troja}, E. and
         {Uchiyama}, Y. and {Yuan}, Y. and {Zimmer}, S.},
        title = "{Minute-timescale \&gt;100 MeV {\ensuremath{\gamma}}-Ray Variability during the Giant Outburst of Quasar 3C 279 Observed by Fermi-LAT in 2015 June}",
      journal = {\apjl},
     keywords = {galaxies: active, galaxies: jets, gamma rays: galaxies, quasars: individual: 3C 279, radiation mechanisms: non-thermal, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = jun,
       volume = {824},
       number = {2},
          eid = {L20},
        pages = {L20},
          doi = {10.3847/2041-8205/824/2/L20},
archivePrefix = {arXiv},
       eprint = {1605.05324},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...824L..20A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2015ApJ...807...79H,
       author = {{Hayashida}, M. and {Nalewajko}, K. and {Madejski}, G.~M. and
         {Sikora}, M. and {Itoh}, R. and {Ajello}, M. and {Blandford}, R.~D. and
         {Buson}, S. and {Chiang}, J. and {Fukazawa}, Y. and {Furniss}, A.~K. and
         {Urry}, C.~M. and {Hasan}, I. and {Harrison}, F.~A. and {Alexand
        er}, D.~M. and {Balokovi{\'c}}, M. and {Barret}, D. and {Boggs}, S.~E. and
         {Christensen}, F.~E. and {Craig}, W.~W. and {Forster}, K. and
         {Giommi}, P. and {Grefenstette}, B. and {Hailey}, C. and
         {Hornstrup}, A. and {Kitaguchi}, T. and {Koglin}, J.~E. and
         {Madsen}, K.~K. and {Mao}, P.~H. and {Miyasaka}, H. and {Mori}, K. and
         {Perri}, M. and {Pivovaroff}, M.~J. and {Puccetti}, S. and {Rana}, V. and
         {Stern}, D. and {Tagliaferri}, G. and {Westergaard}, N.~J. and
         {Zhang}, W.~W. and {Zoglauer}, A. and {Gurwell}, M.~A. and
         {Uemura}, M. and {Akitaya}, H. and {Kawabata}, K.~S. and
         {Kawaguchi}, K. and {Kanda}, Y. and {Moritani}, Y. and {Takaki}, K. and
         {Ui}, T. and {Yoshida}, M. and {Agarwal}, A. and {Gupta}, A.~C.},
        title = "{Rapid Variability of Blazar 3C 279 during Flaring States in 2013-2014 with Joint Fermi-LAT, NuSTAR, Swift, and Ground-Based Multiwavelength Observations}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: jets, gamma rays: galaxies, quasars: individual: 3C 279, radiation mechanisms: non-thermal, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = jul,
       volume = {807},
       number = {1},
          eid = {79},
        pages = {79},
          doi = {10.1088/0004-637X/807/1/79},
archivePrefix = {arXiv},
       eprint = {1502.04699},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...807...79H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Mannheim:1998wp,
      author         = "Mannheim, Karl and Protheroe, R. J. and Rachen, Jorg P.",
      title          = "{On the cosmic ray bound for models of extragalactic
                        neutrino production}",
      journal        = "Phys. Rev.",
      volume         = "D63",
      year           = "2001",
      pages          = "023003",
      doi            = "10.1103/PhysRevD.63.023003",
      eprint         = "astro-ph/9812398",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/9812398;%%"
}
@article{Waxman:1998yy,
      author         = "Waxman, Eli and Bahcall, John N.",
      title          = "{High-energy neutrinos from astrophysical sources: An
                        Upper bound}",
      journal        = "Phys. Rev.",
      volume         = "D59",
      year           = "1999",
      pages          = "023002",
      doi            = "10.1103/PhysRevD.59.023002",
      eprint         = "hep-ph/9807282",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IASSNS-AST-98-38",
      SLACcitation   = "%%CITATION = HEP-PH/9807282;%%"
}
@article{PhysRev.46.76.2,
  title = {Remarks on Super-Novae and Cosmic Rays},
  author = {Baade, W. and Zwicky, F.},
  journal = {Phys. Rev.},
  volume = {46},
  issue = {1},
  pages = {76--77},
  numpages = {0},
  year = {1934},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.46.76.2},
  url = {https://link.aps.org/doi/10.1103/PhysRev.46.76.2}
}
@ARTICLE{1984ARA&A..22..425H,
       author = {{Hillas}, A.~M.},
        title = "{The Origin of Ultra-High-Energy Cosmic Rays}",
      journal = {\araa},
         year = "1984",
        month = "Jan",
       volume = {22},
        pages = {425-444},
          doi = {10.1146/annurev.aa.22.090184.002233},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984ARA&A..22..425H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Gross:2010qma,
      author         = "Gross, Eilam and Vitells, Ofer",
      title          = "{Trial factors for the look elsewhere effect in high
                        energy physics}",
      journal        = "Eur. Phys. J.",
      volume         = "C70",
      year           = "2010",
      pages          = "525-530",
      doi            = "10.1140/epjc/s10052-010-1470-8",
      eprint         = "1005.1891",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.data-an",
      SLACcitation   = "%%CITATION = ARXIV:1005.1891;%%"
}

@article{aartsen2013first,
  title={First observation of PeV-energy neutrinos with IceCube},
  author={Aartsen, M.G. and others},
  journal={Physical review letters},
  volume={111},
  number={2},
  pages={021103},
  year={2013},
  publisher={APS}
}
@article{Aartsen:2013jdh,
      author         = "Aartsen, M. G. and others",
      title          = "{Evidence for High-Energy Extraterrestrial Neutrinos at
                        the IceCube Detector}",
      collaboration  = "IceCube",
      journal        = "Science",
      volume         = "342",
      year           = "2013",
      pages          = "1242856",
      doi            = "10.1126/science.1242856",
      eprint         = "1311.5238",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1311.5238;%%"
}
@article{BRAUN2010175,
title = "Time-dependent point source search methods in high energy neutrino astronomy",
journal = "Astroparticle Physics",
volume = "33",
number = "3",
pages = "175 - 181",
year = "2010",
issn = "0927-6505",
doi = "https://doi.org/10.1016/j.astropartphys.2010.01.005",
url = "http://www.sciencedirect.com/science/article/pii/S0927650510000241",
author = "Jim Braun and Mike Baker and Jon Dumm and Chad Finley and Albrecht Karle and Teresa Montaruli",
keywords = "Neutrino, Point source, Flare, Burst, Search method",
}
@article{Aartsen_2013,
	doi = {10.1088/0004-637x/779/2/132},
	year = {2013},
	month = {dec},
	publisher = {{IOP}, Publishing},
	volume = {779},
	number = {2},
	pages = {132},
	author = {Aartsen, M. G. and others},
	title = {Search for time-independent neutrino emission from astrophysical sources with 3 yr of IceCube data},
	journal = {The Astrophysical Journal}
}

@ARTICLE{2019arXiv191006006U,
       author = {Uro\v{s}evi\'c, Dejan and Arbutina, Bojan and
         Oni\'c, Du\v{s}an},
        title = "{Particle acceleration in interstellar shocks}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Oct",
          eid = {arXiv:1910.06006},
        pages = {arXiv:1910.06006},
archivePrefix = {arXiv},
       eprint = {1910.06006},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv191006006U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2012APh....35..660K,
       author = {{Kampert}, Karl-Heinz and {Unger}, Michael},
        title = "{Measurements of the cosmic ray composition with air shower experiments}",
      journal = {Astroparticle Physics},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = may,
       volume = {35},
       number = {10},
        pages = {660-678},
          doi = {10.1016/j.astropartphys.2012.02.004},
archivePrefix = {arXiv},
       eprint = {1201.0018},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012APh....35..660K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{Fermitools,
author = "{The Fermi Collaboration}",
title = "{Fermi Science Tools v9r31}",
note = "{\url{https://fermi.gsfc.nasa.gov/ssc/data/analysis/documentation/}}"
}

@article{bell1978acceleration,
  title={The acceleration of cosmic rays in shock fronts--I},
  author={Bell, A.R.},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={182},
  number={2},
  pages={147--156},
  year={1978},
  publisher={Oxford University Press Oxford, UK}
}

@article{Aartsen:2016nxy,
      author         = "Aartsen, M. G. and others",
      title          = "{The IceCube Neutrino Observatory: Instrumentation and
                        Online Systems}",
      collaboration  = "IceCube",
      journal        = "JINST",
      volume         = "12",
      year           = "2017",
      number         = "03",
      pages          = "P03012",
      doi            = "10.1088/1748-0221/12/03/P03012",
      eprint         = "1612.05093",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      SLACcitation   = "%%CITATION = ARXIV:1612.05093;%%"
}

@article{Abbasi:2010vc,
    author = "Abbasi, R. and others",
    archivePrefix = "arXiv",
    collaboration = "IceCube",
    doi = "10.1016/j.nima.2010.03.102",
    eprint = "1002.2442",
    journal = "Nucl. Instrum. Meth. A",
    pages = "139--152",
    primaryClass = "astro-ph.IM",
    title = "{Calibration and Characterization of the IceCube Photomultiplier Tube}",
    volume = "618",
    year = "2010"
}

@article{Abbasi:2008aa,
      author         = "Abbasi, R. and others",
      title          = "{The IceCube Data Acquisition System: Signal Capture,
                        Digitization, and Timestamping}",
      collaboration  = "IceCube",
      journal        = "Nucl. Instrum. Meth.",
      volume         = "A601",
      year           = "2009",
      pages          = "294-316",
      doi            = "10.1016/j.nima.2009.01.001",
      eprint         = "0810.4930",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:0810.4930;%%"
}
@article{Schlickeiser,
author = {Schlickeiser, Reinhard},
year = {1988},
month = {12},
pages = {243-293},
title = {Cosmic-ray transport and acceleration. I - Derivation of the kinetic equation and application to cosmic rays in static cold media. II - Cosmic rays in moving cold media with application to diffusive shock wave acceleration},
volume = {336},
journal = {The Astrophysical Journal},
doi = {10.1086/167009}
}

@inproceedings{aller1987evidence,
  title={Evidence for shocks in relativistic jets},
  author={Aller, Hugh D and Hughes, Philip A and Aller, Margo F},
  booktitle={Superluminal Radio Sources},
  pages={273--279},
  editor={{Zensus}, J. Anton and {Pearson}, Timothy J.},
  year={1987}
}

@article{1990Ap&SS.171...13K,
       author = {{Kidger}, M.~R. and {Garcia Lario}, P. and {de Diego}, J.~A.},
        title = "{Visible and near-infrared monitoring of 3C 279 in 1988 1989}",
      journal = {Astrophysics \& Space Science (\apss)},
     keywords = {Astronomical Spectroscopy, Charge Coupled Devices, Galactic Structure, Light Curve, Near Infrared Radiation, Telescopes, Annual Variations, Stellar Luminosity, Visible Spectrum, Astrophysics},
         year = "1990",
        month = "Sep",
       volume = {171},
       number = {1-2},
        pages = {13-15},
          doi = {10.1007/BF00646813},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990Ap&SS.171...13K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2018arXiv181107979I,
       author = { {Aartsen}, M.~G. and others},
        title = "{Search for steady point-like sources in the astrophysical muon neutrino flux with 8 years of IceCube data}",
      journal = {arXiv e-prints},
     keywords = {High Energy Physics - Phenomenology, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2018",
        month = "Nov",
          eid = {arXiv:1811.07979},
        pages = {arXiv:1811.07979},
archivePrefix = {arXiv},
       eprint = {1811.07979},
 primaryClass = {hep-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv181107979I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{1989ApJ...347L...9M,
       author = {{Makino}, F. and {Kii}, T. and {Hayashida}, K. and {Inoue}, H. and
         {Tanaka}, Y. and {Ohashi}, T. and {Makishima}, K. and {Awaki}, H. and
         {Koyama}, K. and {Turner}, M.~J.~L. and {Williams}, O.~R.},
        title = "{X-Ray Outburst of the Quasar 3C 279}",
      journal = {\apjl},
     keywords = {Quasars, X Ray Sources, Astronomical Spectroscopy, Gravitational Effects, Hubble Constant, X Ray Spectra, Astrophysics, GALAXIES: JETS, QUASARS, X-RAYS: SOURCES, X-RAYS: SPECTRA},
         year = "1989",
        month = "Dec",
       volume = {347},
        pages = {L9},
          doi = {10.1086/185594},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1989ApJ...347L...9M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{PhysRevD.75.043006,
  title = {Calculation of atmospheric neutrino flux using the interaction model calibrated with atmospheric muon data},
  author = {Honda, M. and Kajita, T. and Kasahara, K. and Midorikawa, S. and Sanuki, T.},
  journal = {Phys. Rev. D},
  volume = {75},
  issue = {4},
  pages = {043006},
  numpages = {26},
  year = {2007},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.75.043006},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.75.043006}
}

@article{GAISSER2012801,
title = "Spectrum of cosmic-ray nucleons, kaon production, and the atmospheric muon charge ratio",
journal = "Astroparticle Physics",
volume = "35",
number = "12",
pages = "801 - 806",
year = "2012",
issn = "0927-6505",
doi = "https://doi.org/10.1016/j.astropartphys.2012.02.010",
url = "http://www.sciencedirect.com/science/article/pii/S0927650512000497",
author = "Thomas K. Gaisser",
keywords = "Cosmic rays, Muons, Neutrinos",
abstract = "Interpretation of measurements of the muon charge ratio in the TeV range depends on the spectra of protons and neutrons in the primary cosmic radiation and on the inclusive cross sections for production of π± and K± in the atmosphere. Recent measurements of the spectra of cosmic-ray nuclei are used here to estimate separately the energy spectra of protons and neutrons and hence to calculate the charge separated hadronic cascade in the atmosphere. From the corresponding production spectra of μ+ and μ− the μ+/μ− ratio is calculated and compared to recent measurements. The comparison leads to a determination of the relative contribution of kaons and pions. Implications for the spectra of νμ and ν¯μ are discussed."
}

@article{Aartsen:2013eka,
      author         = "Aartsen, M. G. and others",
      title          = "{Search for a diffuse flux of astrophysical muon
                        neutrinos with the IceCube 59-string configuration}",
      collaboration  = "IceCube",
      journal        = "Phys. Rev.",
      volume         = "D89",
      year           = "2014",
      number         = "6",
      pages          = "062007",
      doi            = "10.1103/PhysRevD.89.062007",
      eprint         = "1311.7048",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1311.7048;%%"
}

@article{IceCube:2018dnn,
      author         = "Aartsen, M. G. and others",
      title          = "{Multimessenger observations of a flaring blazar
                        coincident with high-energy neutrino IceCube-170922A}",
      collaboration  = "IceCube, Fermi-LAT, MAGIC, AGILE, ASAS-SN, HAWC,
                        H.E.S.S., INTEGRAL, Kanata, Kiso, Kapteyn, Liverpool
                        Telescope, Subaru, Swift NuSTAR, VERITAS, VLA/17B-403",
      journal        = "Science",
      volume         = "361",
      year           = "2018",
      number         = "6398",
      pages          = "eaat1378",
      doi            = "10.1126/science.aat1378",
      eprint         = "1807.08816",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1807.08816;%%"
}


@article{IceCube:2018cha,
      author         = "Aartsen, M. G. and others",
      title          = "{Neutrino emission from the direction of the blazar TXS
                        0506+056 prior to the IceCube-170922A alert}",
      collaboration  = "IceCube",
      journal        = "Science",
      volume         = "361",
      year           = "2018",
      number         = "6398",
      pages          = "147-151",
      doi            = "10.1126/science.aat2890",
      eprint         = "1807.08794",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1807.08794;%%"
}
@article{Aartsen:2015wto,
      author         = "Aartsen, M. G. and others",
      title          = "{Searches for Time Dependent Neutrino Sources with
                        IceCube Data from 2008 to 2012}",
      collaboration  = "IceCube",
      journal        = "Astrophys. J.",
      volume         = "807",
      year           = "2015",
      number         = "1",
      pages          = "46",
      doi            = "10.1088/0004-637X/807/1/46",
      eprint         = "1503.00598",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1503.00598;%%"
}
@article{aartsen2015atmospheric,
  title={Atmospheric and astrophysical neutrinos above 1 TeV interacting in IceCube},
  author={Aartsen, M. G. and others},
  journal={Physical Review D},
  volume={91},
  number={2},
  pages={022001},
  year={2015},
  publisher={APS}
}
@article{aartsen2017icecube,
  title={The IceCube realtime alert system},
  author={Aartsen, M. G. and others},
  journal={Astroparticle Physics},
  volume={92},
  pages={30--41},
  year={2017},
  publisher={Elsevier}
}
https://www.overleaf.com/project/5c40b5044e3521578a21a88d
@article{aartsen2014searches,
  title={Searches for extended and point-like neutrino sources with four years of IceCube data},
  author={Aartsen, M. G. and others},
  journal={The Astrophysical Journal},
  volume={796},
  number={2},
  pages={109},
  year={2014},
  publisher={IOP Publishing}
}
@article{braun2008methods,
  title={Methods for point source analysis in high energy neutrino telescopes},
  author={Braun, Jim and Dumm, Jon and De Palma, Francesco and Finley, Chad and Karle, Albrecht and Montaruli, Teresa},
  journal={Astroparticle Physics},
  volume={29},
  number={4},
  pages={299--305},
  year={2008},
  publisher={Elsevier}
}
@article{braun2010time,
  title={Time-dependent point source search methods in high energy neutrino astronomy},
  author={Braun, Jim and Baker, Mike and Dumm, Jon and Finley, Chad and Karle, Albrecht and Montaruli, Teresa},
  journal={Astroparticle Physics},
  volume={33},
  number={3},
  pages={175--181},
  year={2010},
  publisher={Elsevier}
}

@ARTICLE{aartsen2017all,
       author = {{Aartsen}, M.~G. and others},
        title = "{All-sky Search for Time-integrated Neutrino Emission from Astrophysical Sources with 7 yr of IceCube Data}",
      journal = {\apj},
     keywords = {astroparticle physics, galaxies: active, neutrinos, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2017",
        month = "Feb",
       volume = {835},
       number = {2},
          eid = {151},
        pages = {151},
          doi = {10.3847/1538-4357/835/2/151},
archivePrefix = {arXiv},
       eprint = {1609.04981},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...835..151A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Abbasi_2011,
	doi = {10.1088/0004-637x/732/1/18},
	year = 2011,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {732},
	number = {1},
	pages = {18},
	author = {Abbasi, R. and others},
	title = {{TIME}-{INTEGRATED} {SEARCHES} {FOR} {POINT}-{LIKE} {SOURCES} {OF} {NEUTRINOS} {WITH} {THE} 40-{STRING} {IceCube} {DETECTOR}},
	journal = {The Astrophysical Journal}
}

@article{abbasi2011time,
  title={Time-dependent searches for point sources of neutrinos with the 40-string and 22-string configurations of IceCube},
  author={Abbasi, R. and others},
  journal={The Astrophysical Journal},
  volume={744},
  number={1},
  pages={1},
  year={2011},
  publisher={IOP Publishing}
}
@article{hartman1992detection,
  title={Detection of high-energy gamma radiation from quasar 3C 279 by the EGRET telescope on the Compton Gamma Ray Observatory},
  author={Hartman, RC and Bertsch, DL and Fichtel, CE and Hunter, SD and Kanbach, G and Kniffen, DA and Kwok, PW and Lin, YC and Mattox, JR and Mayer-Hasselwander, HA and others},
  journal={The Astrophysical Journal},
  volume={385},
  pages={L1--L4},
  year={1992}
}
@article{maraschi1992jet,
  title={A jet model for the gamma-ray emitting blazar 3C 279},
  author={Maraschi, L and Ghisellini, G and Celotti, A},
  journal={The Astrophysical Journal},
  volume={397},
  pages={L5--L9},
  year={1992}
}
@article{wehrle1998multiwavelength,
  title={Multiwavelength observations of a dramatic high-energy flare in the blazar 3C 279},
  author={Wehrle, Ann E and Pian, E and Urry, CM and Maraschi, L and McHardy, IM and Lawson, AJ and Ghisellini, G and Hartman, RC and Madejski, GM and Makino, F and others},
  journal={The Astrophysical Journal},
  volume={497},
  number={1},
  pages={178},
  year={1998},
  publisher={IOP Publishing}
}

@article{gammarays3C279MAGIC2009,
      author         = "Errando, M. and others",
      title          = "{Discovery of very high energy gamma-rays from the flat
                        spectrum radio quasar 3C 279 with the MAGIC telescope}",
      booktitle      = "{Proceedings, 4th Heidelberg International Symposium on
                        High-Energy Gamma Ray Astronomy: Heidelberg, Germany, July
                        7-11, 2008}",
      collaboration  = "MAGIC",
      journal        = "AIP Conf. Proc.",
      volume         = "1085",
      year           = "2009",
      number         = "1",
      pages          = "423-426",
      doi            = "10.1063/1.3076698",
      eprint         = "0901.3275",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:0901.3275;%%"
}

@article{Diltz_2015,
	doi = {10.1088/0004-637x/802/2/133},
	url = {https://doi.org/10.1088%2F0004-637x%2F802%2F2%2F133},
	year = 2015,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {802},
	number = {2},
	pages = {133},
	author = {C. Diltz and M. Böttcher and G. Fossati},
	title = {{TIME} {DEPENDENT} {HADRONIC} {MODELING} {OF} {FLAT} {SPECTRUM} {RADIO} {QUASARS}},
	journal = {The Astrophysical Journal},
}

@article{teshima2007discovery,
      author         = "Teshima, Masahiro and others",
      title          = "{Discovery of Very High Energy Gamma-Rays from the
                        Distant Flat Spectrum Radio Quasar 3C 279 with the MAGIC
                        Telescope}",
      collaboration  = "MAGIC",
      volume         = "3",
      year           = "2007",
      pages          = "1045",
      eprint         = "0709.1475",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "MPP-2007-111",
      SLACcitation   = "%%CITATION = ARXIV:0709.1475;%%"
}

@inproceedings{turler2012multiple,
  title={Multiple synchrotron self-Compton modeling of gamma-ray flares in 3C 279},
  author={T{\"u}rler, Marc and Bj{\"o}rnsson, Claes-Ingvar},
  booktitle={Journal of Physics: Conference Series},
  volume={355},
  number={1},
  pages={012033},
  year={2012},
  organization={IOP Publishing}
}

@article{paliya2016lepto,
  title={Lepto-Hadronic Origin of $\gamma$-ray Outbursts of 3C 279},
  author={Paliya, Vaidehi S and Diltz, Chris and Bottcher, Markus and Stalin, CS and Buckley, David},
  journal={arXiv preprint arXiv:1603.05506},
  year={2016}
}

@article{ackermann2016minute,
      author         = "Ackermann, M. and others",
      title          = "{Minute-Timescale >100 MeV gamma-ray variability during
                        the giant outburst of quasar 3C 279 observed by Fermi-LAT
                        in 2015 June}",
      collaboration  = "Fermi-LAT",
      journal        = "Astrophys. J.",
      volume         = "824",
      year           = "2016",
      number         = "2",
      pages          = "L20",
      doi            = "10.3847/2041-8205/824/2/L20",
      eprint         = "1605.05324",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1605.05324;%%"
}

@article{Aartsen:2019fau,
      author         = "Aartsen, M. G. and others",
      title          = "{Time-integrated Neutrino Source Searches with 10 years of IceCube Data}",
      collaboration  = "IceCube",
      year           = "2019",
      eprint         = "1910.08488",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1910.08488;%%"
}
@article{Ghisellini:2012hs,
      author         = "Ghisellini, Gabriele",
      title          = "{Radiative Processes in High Energy Astrophysics}",
      journal        = "Lect. Notes Phys.",
      volume         = "873",
      year           = "2013",
      pages          = "1-147",
      doi            = "10.1007/978-3-319-00612-3",
      eprint         = "1202.5949",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1202.5949;%%"
}
@INPROCEEDINGS{2019ICRC...36..209C,
       author = {{Caprioli}, D. and {Haggerty}, C.},
        title = "{The Issue with Diffusive Shock Acceleration}",
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Physics - Plasma Physics, Physics - Space Physics},
    booktitle = {36th International Cosmic Ray Conference (ICRC2019)},
         year = "2019",
       series = {International Cosmic Ray Conference},
       volume = {36},
        month = "Jul",
          eid = {209},
        pages = {209},
archivePrefix = {arXiv},
       eprint = {1909.06288},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ICRC...36..209C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Blandford:1987pw,
      author         = "Blandford, R. and Eichler, D.",
      title          = "{Particle Acceleration at Astrophysical Shocks: A Theory
                        of Cosmic Ray Origin}",
      journal        = "Phys. Rept.",
      volume         = "154",
      year           = "1987",
      pages          = "1-75",
      doi            = "10.1016/0370-1573(87)90134-7",
      SLACcitation   = "%%CITATION = PRPLC,154,1;%%"
}
@ARTICLE{2015ATel76331C,
   author = {{Cutini}, S.},
    title = "{Fermi LAT detection of renewed and strong GeV activity from blazar 3C 279}",
  journal = {The Astronomer's Telegram},
 keywords = {Request for Observations, AGN, Blazar, Quasar},
     year = 2015,
    month = jun,
   volume = 7633,
   adsurl = {http://adsabs.harvard.edu/abs/2015ATel.7633....1C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{scargle2013studies,
  title={Studies in astronomical time series analysis. VI. Bayesian block representations},
  author={Scargle, Jeffrey D and Norris, Jay P and Jackson, Brad and Chiang, James},
  journal={The Astrophysical Journal},
  volume={764},
  number={2},
  pages={167},
  year={2013},
  publisher={IOP Publishing}
}
@article{resconi2009classification,
  title={The classification of flaring states of blazars},
  author={Resconi, E and Franco, D and Gross, A and Costamante, L and Flaccomio, E},
  journal={Astronomy \& Astrophysics},
  volume={502},
  number={2},
  pages={499--504},
  year={2009},
  publisher={EDP Sciences}
}
@article{halzen2016high,
  title={High-energy Neutrinos from Recent Blazar Flares},
  author={Halzen, Francis and Kheirandish, Ali},
  journal={The Astrophysical Journal},
  volume={831},
  number={1},
  pages={12},
  year={2016},
  publisher={IOP Publishing}
}

@article{Neunhoffer:2004ha,
      author         = "Neunhoffer, Till",
      title          = "{Estimating the angular resolution of tracks in neutrino
                        telescopes based on a likelihood analysis}",
      journal        = "Astropart. Phys.",
      volume         = "25",
      year           = "2006",
      pages          = "220-225",
      doi            = "10.1016/j.astropartphys.2006.01.002",
      eprint         = "astro-ph/0403367",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0403367;%%"
}

@article{Halzen:2005pz,
      author         = "Halzen, Francis and Hooper, Dan",
      title          = "{High energy neutrinos from the TeV blazar 1ES 1959+650}",
      journal        = "Astropart. Phys.",
      volume         = "23",
      year           = "2005",
      pages          = "537-542",
      doi            = "10.1016/j.astropartphys.2005.03.007",
      eprint         = "astro-ph/0502449",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "MADPH-05-1415",
      SLACcitation   = "%%CITATION = ASTRO-PH/0502449;%%"
}

@article{Atwood:2013rka,
author = {Atwood, W. and Albert, A. and Baldini, L. and Tinivella, Marco and Bregeon, J. and Pesce Rollins, Melissa and Sgrò, C. and Bruel, P. and Charles, E. and Drlica-Wagner, A. and Franckowiak, Anna and Jogler, T. and Rochester, L. and Usher, T. and Wood, M. and Cohen‐Tanugi, Johann and Zimmer, Stephan},
year = {2013},
month = {03},
pages = {},
title = {Pass 8: Toward the Full Realization of the Fermi-LAT Scientific Potential}
}

@article{Aartsen_2016,
	doi = {10.3847/2041-8205/824/2/l28},
	url = {https://doi.org/10.3847%2F2041-8205%2F824%2F2%2Fl28},
	year = 2016,
	month = {jun},
	publisher = {American Astronomical Society},
	volume = {824},
	number = {2},
	pages = {L28},
	author = {M. G. Aartsen and K. Abraham and M. Ackermann and J. Adams and J. A. Aguilar and M. Ahlers and M. Ahrens and D. Altmann and K. Andeen and T. Anderson and I. Ansseau and G. Anton and M. Archinger and C. Arguelles and T. C. Arlen and J. Auffenberg and X. Bai and S. W. Barwick and V. Baum and R. Bay and J. J. Beatty and J. Becker Tjus and K.-H. Becker and S. BenZvi and P. Berghaus and D. Berley and E. Bernardini and A. Bernhard and D. Z. Besson and G. Binder and D. Bindig and M. Bissok and E. Blaufuss and S. Blot and D. J. Boersma and C. Bohm and M. Börner and F. Bos and D. Bose and S. Böser and O. Botner and J. Braun and L. Brayeur and H.-P. Bretz and A. Burgman and N. Buzinsky and J. Casey and M. Casier and E. Cheung and D. Chirkin and A. Christov and K. Clark and L. Classen and S. Coenders and G. H. Collin and J. M. Conrad and D. F. Cowen and A. H. Cruz Silva and J. Daughhetee and J. C. Davis and M. Day and J. P. A. M. de Andr{\'{e}} and C. De Clercq and E. del Pino Rosendo and H. Dembinski and S. De Ridder and P. Desiati and K. D. de Vries and G. de Wasseige and M. de With and T. DeYoung and J. C. D{\'{\i}}az-V{\'{e}}lez and V. di Lorenzo and H. Dujmovic and J. P. Dumm and M. Dunkman and B. Eberhardt and T. Ehrhardt and B. Eichmann and S. Euler and P. A. Evenson and S. Fahey and A. R. Fazely and J. Feintzeig and J. Felde and K. Filimonov and C. Finley and S. Flis and C.-C. Fösig and T. Fuchs and T. K. Gaisser and R. Gaior and J. Gallagher and L. Gerhardt and K. Ghorbani and L. Gladstone and M. Glagla and T. Glüsenkamp and A. Goldschmidt and G. Golup and J. G. Gonzalez and D. G{\'{o}}ra and D. Grant and Z. Griffith and C. Ha and C. Haack and A. Haj Ismail and A. Hallgren and F. Halzen and E. Hansen and B. Hansmann and T. Hansmann and K. Hanson and D. Hebecker and D. Heereman and K. Helbing and R. Hellauer and S. Hickford and J. Hignight and G. C. Hill and K. D. Hoffman and R. Hoffmann and K. Holzapfel and A. Homeier and K. Hoshina and F. Huang and M. Huber and W. Huelsnitz and K. Hultqvist and S. In and A. Ishihara and E. Jacobi and G. S. Japaridze and M. Jeong and K. Jero and B. J. P. Jones and M. Jurkovic and A. Kappes and T. Karg and A. Karle and U. Katz and M. Kauer and A. Keivani and J. L. Kelley and J. Kemp and A. Kheirandish and M. Kim and T. Kintscher and J. Kiryluk and S. R. Klein and G. Kohnen and R. Koirala and H. Kolanoski and R. Konietz and L. Köpke and C. Kopper and S. Kopper and D. J. Koskinen and M. Kowalski and K. Krings and M. Kroll and G. Krückl and C. Krüger and J. Kunnen and S. Kunwar and N. Kurahashi and T. Kuwabara and M. Labare and J. L. Lanfranchi and M. J. Larson and D. Lennarz and M. Lesiak-Bzdak and M. Leuermann and J. Leuner and L. Lu and J. Lünemann and J. Madsen and G. Maggi and K. B. M. Mahn and S. Mancina and M. Mandelartz and R. Maruyama and K. Mase and H. S. Matis and R. Maunu and F. McNally and K. Meagher and M. Medici and M. Meier and A. Meli and T. Menne and G. Merino and T. Meures and S. Miarecki and E. Middell and L. Mohrmann and T. Montaruli and R. Nahnhauer and U. Naumann and G. Neer and H. Niederhausen and S. C. Nowicki and D. R. Nygren and A. Obertacke Pollmann and A. Olivas and A. Omairat and A. O'Murchadha and T. Palczewski and H. Pandya and D. V. Pankova and Ö. Penek and J. A. Pepper and C. P{\'{e}}rez de los Heros and C. Pfendner and D. Pieloth and E. Pinat and J. Posselt and P. B. Price and G. T. Przybylski and M. Quinnan and C. Raab and L. Rädel and M. Rameez and K. Rawlins and R. Reimann and M. Relich and E. Resconi and W. Rhode and M. Richman and B. Riedel and S. Robertson and M. Rongen and C. Rott and T. Ruhe and D. Ryckbosch and L. Sabbatini and A. Sandrock and J. Sandroos and S. Sarkar and K. Satalecka and M. Schimp and P. Schlunder and T. Schmidt and S. Schoenen and S. Schöneberg and A. Schönwald and L. Schumacher and D. Seckel and S. Seunarine and D. Soldin and M. Song and G. M. Spiczak and C. Spiering and M. Stahlberg and M. Stamatikos and T. Stanev and A. Stasik and A. Steuer and T. Stezelberger and R. G. Stokstad and A. Stö{\ss}l and R. Ström and N. L. Strotjohann and G. W. Sullivan and M. Sutherland and H. Taavola and I. Taboada and J. Tatar and S. Ter-Antonyan and A. Terliuk and G. Te{\v{s}}i{\'{c}} and S. Tilav and P. A. Toale and M. N. Tobin and S. Toscano and D. Tosi and M. Tselengidou and A. Turcati and E. Unger and M. Usner and S. Vallecorsa and J. Vandenbroucke and N. van Eijndhoven and S. Vanheule and M. van Rossem and J. van Santen and J. Veenkamp and M. Vehring and M. Voge and M. Vraeghe and C. Walck and A. Wallace and M. Wallraff and N. Wandkowsky and Ch. Weaver and C. Wendt and S. Westerhoff and B. J. Whelan and N. Whitehorn and S. Wickmann and K. Wiebe and C. H. Wiebusch and L. Wille and D. R. Williams and L. Wills and H. Wissing and M. Wolf and T. R. Wood and K. Woschnagg and D. L. Xu and X. W. Xu and Y. Xu and J. P. Yanez and G. Yodh and S. Yoshida and M. Zoll and},
	title = {{LOWERING} {ICECUBE}{\textquotesingle}S {ENERGY} {THRESHOLD} {FOR} {POINT} {SOURCE} {SEARCHES} {IN} {THE} {SOUTHERN} {SKY}},
	journal = {The Astrophysical Journal},
	abstract = {Observation of a point source of astrophysical neutrinos would be a “smoking gun” signature of a cosmic-ray accelerator. While IceCube has recently discovered a diffuse flux of astrophysical neutrinos, no localized point source has been observed. Previous IceCube searches for point sources in the southern sky were restricted by either an energy threshold above a few hundred  TeV or poor neutrino angular resolution. Here we present a search for southern sky point sources with greatly improved sensitivities to neutrinos with energies below 100 TeV. By selecting charged-current ν

μ
 interacting inside the detector, we reduce the atmospheric background while retaining efficiency for astrophysical neutrino-induced events reconstructed with sub-degree angular resolution. The new event sample covers three years of detector data and leads to a factor of 10 improvement in sensitivity to point sources emitting below 100 TeV in the southern sky. No statistically significant evidence of point sources was found, and upper limits are set on neutrino emission from individual sources. A posteriori analysis of the highest-energy (∼100 TeV) starting event in the sample found that this event alone represents a 2.8σ deviation from the hypothesis that the data consists only of atmospheric background.}
}

@article{Sikora_2009,
	doi = {10.1088/0004-637x/704/1/38},
	url = {https://doi.org/10.1088%2F0004-637x%2F704%2F1%2F38},
	year = 2009,
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {704},
	number = {1},
	pages = {38--50},
	author = {Marek Sikora and {\L}ukasz Stawarz and Rafa{\l} Moderski and Krzysztof Nalewajko and Greg M. Madejski},
	title = {{CONSTRAINING} {EMISSION} {MODELS} {OF} {LUMINOUS} {BLAZAR} {SOURCES}},
	journal = {The Astrophysical Journal},
	abstract = {Many luminous blazars which are associated with quasar-type active galactic nuclei display broadband spectra characterized by a large luminosity ratio of their high-energy (γ-ray) and low-energy (synchrotron) spectral components. This large ratio, reaching values up to 100, challenges the standard synchrotron self-Compton models by means of substantial departures from the minimum power condition. Luminous blazars also typically have very hard X-ray spectra, and those in turn seem to challenge hadronic scenarios for the high-energy blazar emission. As shown in this paper, no such problems are faced by the models which involve Comptonization of radiation provided by a broad-line region, or dusty molecular torus. The lack or weakness of bulk-Compton and Klein-Nishina features indicated by the presently available data favors the production of γ-rays via upscattering of infrared photons from hot dust. This implies that the blazar emission zone is located at parsec-scale distances from the nucleus, and as such is possibly associated with the extended, quasi-stationary reconfinement shocks formed in relativistic outflows. This scenario predicts characteristic timescales for flux changes in luminous blazars to be days/weeks, consistent with the variability patterns observed in such systems at infrared, optical, and γ-ray frequencies. We also propose that the parsec-scale blazar activity can be occasionally accompanied by dissipative events taking place at sub-parsec distances and powered by internal shocks and/or reconnection of magnetic fields. These could account for the multiwavelength intraday flares occasionally observed in powerful blazar sources.}
}

@article{Abeysekara_2018,
	doi = {10.3847/2041-8213/aad053},
	url = {https://doi.org/10.3847%2F2041-8213%2Faad053},
	year = 2018,
	month = {jul},
	publisher = {American Astronomical Society},
	volume = {861},
	number = {2},
	pages = {L20},
	author = {A. U. Abeysekara and A. Archer and W. Benbow and R. Bird and A. Brill and R. Brose and J. H. Buckley and J. L. Christiansen and A. J. Chromey and M. K. Daniel and A. Falcone and Q. Feng and J. P. Finley and L. Fortson and A. Furniss and G. H. Gillanders and O. Gueta and D. Hanna and O. Hervet and J. Holder and G. Hughes and T. B. Humensky and C. A. Johnson and P. Kaaret and P. Kar and N. Kelley-Hoskins and M. Kertzman and D. Kieda and M. Krause and F. Krennrich and M. J. Lang and P. Moriarty and R. Mukherjee and S. O'Brien and R. A. Ong and A. N. Otte and N. Park and A. Petrashyk and M. Pohl and E. Pueschel and J. Quinn and K. Ragan and P. T. Reynolds and G. T. Richards and E. Roache and C. Rulten and I. Sadeh and M. Santander and S. S. Scott and G. H. Sembroski and K. Shahinyan and J. Tyler and S. P. Wakely and A. Weinstein and R. M. Wells and P. Wilcox and A. Wilhelm and D. A. Williams and T. J Williamson and B. Zitzer and A. Kaur and},
	title = {{VERITAS} Observations of the {BL} Lac Object {TXS} 0506$\mathplus$056},
	journal = {The Astrophysical Journal},
	abstract = {On 2017 September 22, the IceCube Neutrino Observatory reported the detection of the high-energy neutrino event IC 170922A, of potential astrophysical origin. It was soon determined that the neutrino direction was consistent with the location of the gamma-ray blazar TXS 0506+056 (3FGL J0509.4+0541), which was in an elevated gamma-ray emission state as measured by the Fermi satellite. Very Energetic Radiation Imaging Telescope Array System (VERITAS) observations of the neutrino/blazar region started on 2017 September 23 in response to the neutrino alert and continued through 2018 February 6. While no significant very-high-energy (VHE; E > 100 GeV) emission was observed from the blazar by VERITAS in the two-week period immediately following the IceCube alert, TXS 0506+056 was detected by VERITAS with a significance of 5.8 standard deviations (σ) in the full 35 hr data set. The average photon flux of the source during this period was (8.9 ± 1.6) × 10−12 cm−2 s−1, or 1.6% of the Crab Nebula flux, above an energy threshold of 110 GeV, with a soft spectral index of 4.8 ± 1.3.}
}

@article{Oikonomou_2019,
   title={High-energy neutrino flux from individual blazar flares},
   volume={489},
   ISSN={1365-2966},
   url={http://dx.doi.org/10.1093/mnras/stz2246},
   DOI={10.1093/mnras/stz2246},
   number={3},
   journal={Monthly Notices of the Royal Astronomical Society},
   publisher={Oxford University Press (OUP)},
   author={Oikonomou, Foteini and Murase, Kohta and Padovani, Paolo and Resconi, Elisa and Meszaros, Peter},
   year={2019},
   month={Sep},
   pages={4347--4366}
}

@article{Penacchioni_2019,
	doi = {10.3847/2041-8213/ab0087},
	url = {https://doi.org/10.3847%2F2041-8213%2Fab0087},
	year = 2019,
	month = {jan},
	publisher = {American Astronomical Society},
	volume = {871},
	number = {2},
	pages = {L30},
	author = {A. V. Penacchioni and O. Civitarese},
	title = {Time Delay between Neutrinos and Gamma-Rays in Short Gamma-Ray Bursts},
	journal = {The Astrophysical Journal},
	abstract = {In this Letter we make an estimate of the time delay between signals, recorded at detectors on Earth, of neutrinos and photons originated in a short gamma-ray burst. We describe the geometry and dynamics of the system according to the Fireshell model. The delay in the photon’s arrival time is produced because the system is originally opaque to radiation; thus, the photons remain trapped and thermalize until the transparency condition is reached. We calculate the time interval between neutrino emission and photon emission in the black hole frame and transform it to the observer frame using Lorentz transformations. We obtain a difference in the arrival time at Earth of .}
}

@phdthesis{Christov:2016zti,
    author = "Christov, Asen",
    title = "{Multi-Messenger studies with the IceCube Detector}",
    doi = "10.13097/archive-ouverte/unige:91766",
    school = "Geneva U.",
    year = "2016"
}

@article{energyRecoMethods2014,
author = {Aartsen, M. and Ackermann, M. and Adams, J. and Aguilar Sánchez, Juan Antonio and Ahlers, M. and Altmann, David and Arguelles, C. and Auffenberg, J. and Bai, Xiaoqiong and Baker, Moatasem and Barwick, S. and Baum, V. and Bay, Ryan and Beatty, J. and Tjus, J. and Becker, K. and BenZvi, S. and Berghaus, P.},
year = {2014},
month = {03},
pages = {P03009},
title = {Energy Reconstruction Methods in the IceCube Neutrino Telescope},
volume = {9},
journal = {Journal of Instrumentation},
doi = {10.1088/1748-0221/9/03/P03009}
}
